On the geometry of the higher dimensional Voisin maps

Voisin constructed self-rational maps of Calabi-Yau manifolds obtained as varieties of $r$-planes in cubic hypersurfaces of adequate dimension. This map has been thoroughly studied in the case $r=1$, which is the Beauville-Donagi case. In this paper, we compute the action of $\Psi$ on holomorphic forms for any $r$. For $r=2$, we compute the action of $\Psi$ on the Chow group of $0$-cycles, and confirm that it is as expected from the generalized Bloch conjecture.

==> chow_of_F_mathematica_1.tex <==
%% AMS-LaTeX Created with the Wolfram Language : www.wolfram.com


\begin{doublespace}
\noindent\(\pmb{\text{(*Define the variables*)}}\\
\pmb{\text{li} = \text{Array}[l, 3]; \text{(*l1, l2, l3*)}}\\
\pmb{\text{mj} = \text{Array}[m, 6]; \text{(*m1, m2, m3, m4, m5, m6*)}}\\
\pmb{\text{(*Create the product expression*)}}\\
\pmb{\text{productExpr} = \text{Product}[\text{li}[[i]] + \text{mj}[[j]], \{i, 1, 3\}, \{j, 1, 6\}];}\\
\pmb{\text{sym1} = \text{SymmetricReduction}[\text{productExpr}, \text{mj}, \{\text{d1}, \text{d2}, \text{d3}, \text{d4}, \text{d5}, \text{d6}\}][[1]];}\\
\pmb{\text{sym2} = \text{SymmetricReduction}[\text{sym1}, \text{li}, \{\text{c1}, \text{c2}, \text{c3}\}][[1]]}\)
\end{doublespace}

\begin{doublespace}
\noindent\(\text{c3}^6+\text{c2} \text{c3}^5 \text{d1}+\text{c1} \text{c3}^5 (\text{d1}^2-2 \text{d2})+\text{c2}^2 \text{c3}^4 \text{d2}+\text{c1}
\text{c2} \text{c3}^4 (\text{d1} \text{d2}-3 \text{d3})+\text{c2}^3 \text{c3}^3 \text{d3}+\text{c3}^5 (\text{d1}^3-6 \text{d3}+3 (-\text{d1}
\text{d2}+3 \text{d3}))+\text{c1} \text{c2}^2 \text{c3}^3 (\text{d1} \text{d3}-4 \text{d4})+\text{c2}^4 \text{c3}^2 \text{d4}+\text{c1}^2 \text{c3}^4
(\text{d2}^2-6 \text{d4}+2 (-\text{d1} \text{d3}+4 \text{d4}))+\text{c2} \text{c3}^4 (\text{d1}^2 \text{d2}-12 \text{d4}+5 (-\text{d1}
\text{d3}+4 \text{d4})+2 (-\text{d2}^2+6 \text{d4}-2 (-\text{d1} \text{d3}+4 \text{d4})))+\text{c1} \text{c2}^3 \text{c3}^2 (\text{d1}
\text{d4}-5 \text{d5})+\text{c2}^5 \text{c3} \text{d5}+\text{c1}^2 \text{c2} \text{c3}^3 (\text{d2} \text{d3}-10 \text{d5}+3 (-\text{d1} \text{d4}+5
\text{d5}))+\text{c2}^2 \text{c3}^3 (\text{d1}^2 \text{d3}-20 \text{d5}+7 (-\text{d1} \text{d4}+5 \text{d5})+2 (-\text{d2} \text{d3}+10 \text{d5}-3
(-\text{d1} \text{d4}+5 \text{d5})))+\text{c1} \text{c3}^4 (\text{d1} \text{d2}^2-30 \text{d5}+12 (-\text{d1} \text{d4}+5 \text{d5})+5
(-\text{d2} \text{d3}+10 \text{d5}-3 (-\text{d1} \text{d4}+5 \text{d5}))+2 (-\text{d1}^2 \text{d3}+20 \text{d5}-7 (-\text{d1} \text{d4}+5 \text{d5})-2
(-\text{d2} \text{d3}+10 \text{d5}-3 (-\text{d1} \text{d4}+5 \text{d5}))))+\text{c1} \text{c2}^4 \text{c3} (\text{d1} \text{d5}-6 \text{d6})+\text{c2}^6
\text{d6}+\text{c1} \text{c2}^5 \text{d1} \text{d6}+\text{c1}^2 \text{c2}^4 \text{d2} \text{d6}+\text{c1}^3 \text{c2}^3 \text{d3} \text{d6}+\text{c1}^4
\text{c2}^2 \text{d4} \text{d6}+\text{c1}^5 \text{c2} \text{d5} \text{d6}+\text{c1}^6 \text{d6}^2+\text{c1}^5 \text{d1} \text{d6}^2+\text{c1}^4 \text{d2}
\text{d6}^2+\text{c1}^3 \text{d3} \text{d6}^2+\text{c1}^2 \text{d4} \text{d6}^2+\text{c1} \text{d5} \text{d6}^2+\text{d6}^3+\text{c1}^2 \text{c2}^3
\text{c3} (\text{d2} \text{d5}-5 \text{d1} \text{d6})+\text{c1}^3 \text{c2}^2 \text{c3} (\text{d3} \text{d5}-4 \text{d2} \text{d6})+\text{c2}^5 (\text{d1}^2
\text{d6}-2 \text{d2} \text{d6})+\text{c1}^4 \text{c2} \text{c3} (\text{d4} \text{d5}-3 \text{d3} \text{d6})+\text{c1} \text{c2}^4 (\text{d1}
\text{d2} \text{d6}-3 \text{d3} \text{d6})+\text{c1}^2 \text{c2}^3 (\text{d1} \text{d3} \text{d6}-4 \text{d4} \text{d6})+\text{c1}^5 \text{c3} (\text{d5}^2-2
\text{d4} \text{d6})+\text{c1}^3 \text{c2}^2 (\text{d1} \text{d4} \text{d6}-5 \text{d5} \text{d6})+\text{c1}^4 \text{c2} (\text{d1} \text{d5}
\text{d6}-6 \text{d6}^2)+\text{c1}^3 \text{c2} (\text{d2} \text{d5} \text{d6}-5 \text{d1} \text{d6}^2)+\text{c1}^2 \text{c2} (\text{d3}
\text{d5} \text{d6}-4 \text{d2} \text{d6}^2)+\text{c1} \text{c2} (\text{d4} \text{d5} \text{d6}-3 \text{d3} \text{d6}^2)+\text{c2}
(\text{d5}^2 \text{d6}-2 \text{d4} \text{d6}^2)+\text{c1}^2 \text{c2}^2 \text{c3}^2 (\text{d2} \text{d4}-15 \text{d6}+4 (-\text{d1} \text{d5}+6
\text{d6}))+\text{c2}^4 \text{c3} (\text{d1}^2 \text{d5}-11 \text{d1} \text{d6}+2 (-\text{d2} \text{d5}+5 \text{d1} \text{d6}))+\text{c1}^3
\text{c2} \text{c3}^2 (\text{d3} \text{d4}-10 \text{d1} \text{d6}+3 (-\text{d2} \text{d5}+5 \text{d1} \text{d6}))+\text{c1}^4 \text{c3}^2 (\text{d4}^2-6
\text{d2} \text{d6}+2 (-\text{d3} \text{d5}+4 \text{d2} \text{d6}))+\text{c1} \text{c2}^3 \text{c3} (\text{d1} \text{d2} \text{d5}-14
\text{d2} \text{d6}+5 (-\text{d1}^2 \text{d6}+2 \text{d2} \text{d6})+3 (-\text{d3} \text{d5}+4 \text{d2} \text{d6}))+\text{c1}^2
\text{c2}^2 \text{c3} (\text{d1} \text{d3} \text{d5}-15 \text{d3} \text{d6}+4 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})+4 (-\text{d1} \text{d2}
\text{d6}+3 \text{d3} \text{d6}))+\text{c2}^4 (\text{d2}^2 \text{d6}-6 \text{d4} \text{d6}+2 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))+\text{c1}^3
\text{c2} \text{c3} (\text{d1} \text{d4} \text{d5}-14 \text{d4} \text{d6}+5 (-\text{d5}^2+2 \text{d4} \text{d6})+3 (-\text{d1} \text{d3}
\text{d6}+4 \text{d4} \text{d6}))+\text{c1}^4 \text{c3} (\text{d1} \text{d5}^2-11 \text{d5} \text{d6}+2 (-\text{d1} \text{d4} \text{d6}+5
\text{d5} \text{d6}))+\text{c1} \text{c2}^3 (\text{d2} \text{d3} \text{d6}-10 \text{d5} \text{d6}+3 (-\text{d1} \text{d4} \text{d6}+5 \text{d5}
\text{d6}))+\text{c1}^2 \text{c2}^2 (\text{d2} \text{d4} \text{d6}-15 \text{d6}^2+4 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2))+\text{c1}
\text{c2}^2 (\text{d3} \text{d4} \text{d6}-10 \text{d1} \text{d6}^2+3 (-\text{d2} \text{d5} \text{d6}+5 \text{d1} \text{d6}^2))+\text{c2}^2
(\text{d4}^2 \text{d6}-6 \text{d2} \text{d6}^2+2 (-\text{d3} \text{d5} \text{d6}+4 \text{d2} \text{d6}^2))+\text{c3} (\text{d5}^3-6
\text{d3} \text{d6}^2+3 (-\text{d4} \text{d5} \text{d6}+3 \text{d3} \text{d6}^2))+\text{c1}^3 \text{c3}^3 (\text{d3}^2-20 \text{d6}+6
(-\text{d1} \text{d5}+6 \text{d6})+2 (-\text{d2} \text{d4}+15 \text{d6}-4 (-\text{d1} \text{d5}+6 \text{d6})))+\text{c2}^3 \text{c3}^2 (\text{d1}^2
\text{d4}-30 \text{d6}+9 (-\text{d1} \text{d5}+6 \text{d6})+2 (-\text{d2} \text{d4}+15 \text{d6}-4 (-\text{d1} \text{d5}+6 \text{d6})))+\text{c1}
\text{c2}^2 \text{c3}^2 (\text{d1} \text{d2} \text{d4}-35 \text{d1} \text{d6}+11 (-\text{d2} \text{d5}+5 \text{d1} \text{d6})+3 (-\text{d3}
\text{d4}+10 \text{d1} \text{d6}-3 (-\text{d2} \text{d5}+5 \text{d1} \text{d6}))+4 (-\text{d1}^2 \text{d5}+11 \text{d1} \text{d6}-2 (-\text{d2}
\text{d5}+5 \text{d1} \text{d6})))+\text{c1}^2 \text{c2} \text{c3}^2 (\text{d1} \text{d3} \text{d4}-32 \text{d2} \text{d6}+10 (-\text{d1}^2
\text{d6}+2 \text{d2} \text{d6})+11 (-\text{d3} \text{d5}+4 \text{d2} \text{d6})+3 (-\text{d1} \text{d2} \text{d5}+14 \text{d2} \text{d6}-5
(-\text{d1}^2 \text{d6}+2 \text{d2} \text{d6})-3 (-\text{d3} \text{d5}+4 \text{d2} \text{d6}))+4 (-\text{d4}^2+6 \text{d2}
\text{d6}-2 (-\text{d3} \text{d5}+4 \text{d2} \text{d6})))+\text{c1}^3 \text{c3}^2 (\text{d1} \text{d4}^2-24 \text{d3} \text{d6}+9
(-\text{d4} \text{d5}+3 \text{d3} \text{d6})+6 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})+2 (-\text{d1} \text{d3} \text{d5}+15 \text{d3}
\text{d6}-4 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-4 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})))+\text{c2}^3 \text{c3} (\text{d2}^2
\text{d5}-24 \text{d3} \text{d6}+6 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})+9 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})+2 (-\text{d1}
\text{d3} \text{d5}+15 \text{d3} \text{d6}-4 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-4 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})))+\text{c1}
\text{c2}^2 \text{c3} (\text{d2} \text{d3} \text{d5}-32 \text{d4} \text{d6}+10 (-\text{d5}^2+2 \text{d4} \text{d6})+11 (-\text{d1}
\text{d3} \text{d6}+4 \text{d4} \text{d6})+3 (-\text{d1} \text{d4} \text{d5}+14 \text{d4} \text{d6}-5 (-\text{d5}^2+2 \text{d4} \text{d6})-3
(-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))+4 (-\text{d2}^2 \text{d6}+6 \text{d4} \text{d6}-2 (-\text{d1} \text{d3} \text{d6}+4
\text{d4} \text{d6})))+\text{c1}^2 \text{c2} \text{c3} (\text{d2} \text{d4} \text{d5}-35 \text{d5} \text{d6}+11 (-\text{d1} \text{d4}
\text{d6}+5 \text{d5} \text{d6})+3 (-\text{d2} \text{d3} \text{d6}+10 \text{d5} \text{d6}-3 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6}))+4
(-\text{d1} \text{d5}^2+11 \text{d5} \text{d6}-2 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6})))+\text{c2}^3 (\text{d3}^2
\text{d6}-20 \text{d6}^2+6 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)+2 (-\text{d2} \text{d4} \text{d6}+15 \text{d6}^2-4 (-\text{d1}
\text{d5} \text{d6}+6 \text{d6}^2)))+\text{c1}^3 \text{c3} (\text{d2} \text{d5}^2-30 \text{d6}^2+9 (-\text{d1} \text{d5}
\text{d6}+6 \text{d6}^2)+2 (-\text{d2} \text{d4} \text{d6}+15 \text{d6}^2-4 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)))+\text{c1}^2
\text{c3} (\text{d3} \text{d5}^2-20 \text{d1} \text{d6}^2+7 (-\text{d2} \text{d5} \text{d6}+5 \text{d1} \text{d6}^2)+2 (-\text{d3}
\text{d4} \text{d6}+10 \text{d1} \text{d6}^2-3 (-\text{d2} \text{d5} \text{d6}+5 \text{d1} \text{d6}^2)))+\text{c1} \text{c3}
(\text{d4} \text{d5}^2-12 \text{d2} \text{d6}^2+5 (-\text{d3} \text{d5} \text{d6}+4 \text{d2} \text{d6}^2)+2 (-\text{d4}^2 \text{d6}+6
\text{d2} \text{d6}^2-2 (-\text{d3} \text{d5} \text{d6}+4 \text{d2} \text{d6}^2)))+\text{c1} \text{c2} \text{c3}^3 (\text{d1}
\text{d2} \text{d3}-60 \text{d6}+22 (-\text{d1} \text{d5}+6 \text{d6})+8 (-\text{d2} \text{d4}+15 \text{d6}-4 (-\text{d1} \text{d5}+6 \text{d6}))+3
(-\text{d1}^2 \text{d4}+30 \text{d6}-9 (-\text{d1} \text{d5}+6 \text{d6})-2 (-\text{d2} \text{d4}+15 \text{d6}-4 (-\text{d1} \text{d5}+6 \text{d6})))+3
(-\text{d3}^2+20 \text{d6}-6 (-\text{d1} \text{d5}+6 \text{d6})-2 (-\text{d2} \text{d4}+15 \text{d6}-4 (-\text{d1} \text{d5}+6 \text{d6}))))+\text{c1}^2
\text{c3}^3 (\text{d1} \text{d3}^2-50 \text{d1} \text{d6}+18 (-\text{d2} \text{d5}+5 \text{d1} \text{d6})+7 (-\text{d3} \text{d4}+10 \text{d1}
\text{d6}-3 (-\text{d2} \text{d5}+5 \text{d1} \text{d6}))+6 (-\text{d1}^2 \text{d5}+11 \text{d1} \text{d6}-2 (-\text{d2} \text{d5}+5 \text{d1}
\text{d6}))+2 (-\text{d1} \text{d2} \text{d4}+35 \text{d1} \text{d6}-11 (-\text{d2} \text{d5}+5 \text{d1} \text{d6})-3 (-\text{d3} \text{d4}+10
\text{d1} \text{d6}-3 (-\text{d2} \text{d5}+5 \text{d1} \text{d6}))-4 (-\text{d1}^2 \text{d5}+11 \text{d1} \text{d6}-2 (-\text{d2} \text{d5}+5
\text{d1} \text{d6}))))+\text{c2}^2 \text{c3}^2 (\text{d2}^2 \text{d4}-53 \text{d2} \text{d6}+20 (-\text{d1}^2 \text{d6}+2
\text{d2} \text{d6})+18 (-\text{d3} \text{d5}+4 \text{d2} \text{d6})+7 (-\text{d1} \text{d2} \text{d5}+14 \text{d2} \text{d6}-5 (-\text{d1}^2
\text{d6}+2 \text{d2} \text{d6})-3 (-\text{d3} \text{d5}+4 \text{d2} \text{d6}))+6 (-\text{d4}^2+6 \text{d2} \text{d6}-2 (-\text{d3}
\text{d5}+4 \text{d2} \text{d6}))+2 (-\text{d1} \text{d3} \text{d4}+32 \text{d2} \text{d6}-10 (-\text{d1}^2 \text{d6}+2 \text{d2}
\text{d6})-11 (-\text{d3} \text{d5}+4 \text{d2} \text{d6})-3 (-\text{d1} \text{d2} \text{d5}+14 \text{d2} \text{d6}-5 (-\text{d1}^2
\text{d6}+2 \text{d2} \text{d6})-3 (-\text{d3} \text{d5}+4 \text{d2} \text{d6}))-4 (-\text{d4}^2+6 \text{d2} \text{d6}-2 (-\text{d3}
\text{d5}+4 \text{d2} \text{d6}))))+\text{c1} \text{c2} \text{c3}^2 (\text{d2} \text{d3} \text{d4}-60 \text{d3} \text{d6}+22
(-\text{d4} \text{d5}+3 \text{d3} \text{d6})+22 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})+8 (-\text{d1} \text{d3} \text{d5}+15 \text{d3}
\text{d6}-4 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-4 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6}))+3 (-\text{d2}^2 \text{d5}+24
\text{d3} \text{d6}-6 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-9 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})-2 (-\text{d1} \text{d3}
\text{d5}+15 \text{d3} \text{d6}-4 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-4 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})))+3
(-\text{d1} \text{d4}^2+24 \text{d3} \text{d6}-9 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-6 (-\text{d1} \text{d2} \text{d6}+3 \text{d3}
\text{d6})-2 (-\text{d1} \text{d3} \text{d5}+15 \text{d3} \text{d6}-4 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-4 (-\text{d1} \text{d2} \text{d6}+3
\text{d3} \text{d6}))))+\text{c1}^2 \text{c3}^2 (\text{d2} \text{d4}^2-53 \text{d4} \text{d6}+20 (-\text{d5}^2+2 \text{d4}
\text{d6})+18 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6})+7 (-\text{d1} \text{d4} \text{d5}+14 \text{d4} \text{d6}-5 (-\text{d5}^2+2
\text{d4} \text{d6})-3 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))+6 (-\text{d2}^2 \text{d6}+6 \text{d4} \text{d6}-2
(-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))+2 (-\text{d2} \text{d3} \text{d5}+32 \text{d4} \text{d6}-10 (-\text{d5}^2+2
\text{d4} \text{d6})-11 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6})-3 (-\text{d1} \text{d4} \text{d5}+14 \text{d4} \text{d6}-5
(-\text{d5}^2+2 \text{d4} \text{d6})-3 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))-4 (-\text{d2}^2 \text{d6}+6
\text{d4} \text{d6}-2 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))))+\text{c2}^2 \text{c3} (\text{d3}^2 \text{d5}-50
\text{d5} \text{d6}+18 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6})+7 (-\text{d2} \text{d3} \text{d6}+10 \text{d5} \text{d6}-3 (-\text{d1}
\text{d4} \text{d6}+5 \text{d5} \text{d6}))+6 (-\text{d1} \text{d5}^2+11 \text{d5} \text{d6}-2 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6}))+2
(-\text{d2} \text{d4} \text{d5}+35 \text{d5} \text{d6}-11 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6})-3 (-\text{d2} \text{d3} \text{d6}+10
\text{d5} \text{d6}-3 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6}))-4 (-\text{d1} \text{d5}^2+11 \text{d5} \text{d6}-2 (-\text{d1}
\text{d4} \text{d6}+5 \text{d5} \text{d6}))))+\text{c1} \text{c2} \text{c3} (\text{d3} \text{d4} \text{d5}-60 \text{d6}^2+22
(-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)+8 (-\text{d2} \text{d4} \text{d6}+15 \text{d6}^2-4 (-\text{d1} \text{d5} \text{d6}+6
\text{d6}^2))+3 (-\text{d2} \text{d5}^2+30 \text{d6}^2-9 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)-2 (-\text{d2}
\text{d4} \text{d6}+15 \text{d6}^2-4 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)))+3 (-\text{d3}^2 \text{d6}+20 \text{d6}^2-6
(-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)-2 (-\text{d2} \text{d4} \text{d6}+15 \text{d6}^2-4 (-\text{d1} \text{d5} \text{d6}+6
\text{d6}^2))))+\text{c2} \text{c3} (\text{d4}^2 \text{d5}-30 \text{d1} \text{d6}^2+12 (-\text{d2} \text{d5} \text{d6}+5
\text{d1} \text{d6}^2)+5 (-\text{d3} \text{d4} \text{d6}+10 \text{d1} \text{d6}^2-3 (-\text{d2} \text{d5} \text{d6}+5 \text{d1} \text{d6}^2))+2
(-\text{d3} \text{d5}^2+20 \text{d1} \text{d6}^2-7 (-\text{d2} \text{d5} \text{d6}+5 \text{d1} \text{d6}^2)-2 (-\text{d3} \text{d4}
\text{d6}+10 \text{d1} \text{d6}^2-3 (-\text{d2} \text{d5} \text{d6}+5 \text{d1} \text{d6}^2))))+\text{c3}^4 (\text{d2}^3-90
\text{d6}+36 (-\text{d1} \text{d5}+6 \text{d6})+15 (-\text{d2} \text{d4}+15 \text{d6}-4 (-\text{d1} \text{d5}+6 \text{d6}))+6 (-\text{d1}^2
\text{d4}+30 \text{d6}-9 (-\text{d1} \text{d5}+6 \text{d6})-2 (-\text{d2} \text{d4}+15 \text{d6}-4 (-\text{d1} \text{d5}+6 \text{d6})))+6 (-\text{d3}^2+20
\text{d6}-6 (-\text{d1} \text{d5}+6 \text{d6})-2 (-\text{d2} \text{d4}+15 \text{d6}-4 (-\text{d1} \text{d5}+6 \text{d6})))+3 (-\text{d1}
\text{d2} \text{d3}+60 \text{d6}-22 (-\text{d1} \text{d5}+6 \text{d6})-8 (-\text{d2} \text{d4}+15 \text{d6}-4 (-\text{d1} \text{d5}+6 \text{d6}))-3
(-\text{d1}^2 \text{d4}+30 \text{d6}-9 (-\text{d1} \text{d5}+6 \text{d6})-2 (-\text{d2} \text{d4}+15 \text{d6}-4 (-\text{d1} \text{d5}+6 \text{d6})))-3
(-\text{d3}^2+20 \text{d6}-6 (-\text{d1} \text{d5}+6 \text{d6})-2 (-\text{d2} \text{d4}+15 \text{d6}-4 (-\text{d1} \text{d5}+6 \text{d6})))))+\text{c2}
\text{c3}^3 (\text{d2}^2 \text{d3}-80 \text{d1} \text{d6}+31 (-\text{d2} \text{d5}+5 \text{d1} \text{d6})+12 (-\text{d3} \text{d4}+10 \text{d1}
\text{d6}-3 (-\text{d2} \text{d5}+5 \text{d1} \text{d6}))+12 (-\text{d1}^2 \text{d5}+11 \text{d1} \text{d6}-2 (-\text{d2} \text{d5}+5 \text{d1}
\text{d6}))+5 (-\text{d1} \text{d2} \text{d4}+35 \text{d1} \text{d6}-11 (-\text{d2} \text{d5}+5 \text{d1} \text{d6})-3 (-\text{d3} \text{d4}+10
\text{d1} \text{d6}-3 (-\text{d2} \text{d5}+5 \text{d1} \text{d6}))-4 (-\text{d1}^2 \text{d5}+11 \text{d1} \text{d6}-2 (-\text{d2} \text{d5}+5
\text{d1} \text{d6})))+2 (-\text{d1} \text{d3}^2+50 \text{d1} \text{d6}-18 (-\text{d2} \text{d5}+5 \text{d1} \text{d6})-7 (-\text{d3}
\text{d4}+10 \text{d1} \text{d6}-3 (-\text{d2} \text{d5}+5 \text{d1} \text{d6}))-6 (-\text{d1}^2 \text{d5}+11 \text{d1} \text{d6}-2 (-\text{d2}
\text{d5}+5 \text{d1} \text{d6}))-2 (-\text{d1} \text{d2} \text{d4}+35 \text{d1} \text{d6}-11 (-\text{d2} \text{d5}+5 \text{d1} \text{d6})-3
(-\text{d3} \text{d4}+10 \text{d1} \text{d6}-3 (-\text{d2} \text{d5}+5 \text{d1} \text{d6}))-4 (-\text{d1}^2 \text{d5}+11 \text{d1} \text{d6}-2
(-\text{d2} \text{d5}+5 \text{d1} \text{d6})))))+\text{c1} \text{c3}^3 (\text{d2} \text{d3}^2-80 \text{d2} \text{d6}+30
(-\text{d1}^2 \text{d6}+2 \text{d2} \text{d6})+31 (-\text{d3} \text{d5}+4 \text{d2} \text{d6})+12 (-\text{d1} \text{d2} \text{d5}+14
\text{d2} \text{d6}-5 (-\text{d1}^2 \text{d6}+2 \text{d2} \text{d6})-3 (-\text{d3} \text{d5}+4 \text{d2} \text{d6}))+12 (-\text{d4}^2+6
\text{d2} \text{d6}-2 (-\text{d3} \text{d5}+4 \text{d2} \text{d6}))+5 (-\text{d1} \text{d3} \text{d4}+32 \text{d2} \text{d6}-10 (-\text{d1}^2
\text{d6}+2 \text{d2} \text{d6})-11 (-\text{d3} \text{d5}+4 \text{d2} \text{d6})-3 (-\text{d1} \text{d2} \text{d5}+14 \text{d2} \text{d6}-5
(-\text{d1}^2 \text{d6}+2 \text{d2} \text{d6})-3 (-\text{d3} \text{d5}+4 \text{d2} \text{d6}))-4 (-\text{d4}^2+6 \text{d2}
\text{d6}-2 (-\text{d3} \text{d5}+4 \text{d2} \text{d6})))+2 (-\text{d2}^2 \text{d4}+53 \text{d2} \text{d6}-20 (-\text{d1}^2
\text{d6}+2 \text{d2} \text{d6})-18 (-\text{d3} \text{d5}+4 \text{d2} \text{d6})-7 (-\text{d1} \text{d2} \text{d5}+14 \text{d2} \text{d6}-5
(-\text{d1}^2 \text{d6}+2 \text{d2} \text{d6})-3 (-\text{d3} \text{d5}+4 \text{d2} \text{d6}))-6 (-\text{d4}^2+6 \text{d2}
\text{d6}-2 (-\text{d3} \text{d5}+4 \text{d2} \text{d6}))-2 (-\text{d1} \text{d3} \text{d4}+32 \text{d2} \text{d6}-10 (-\text{d1}^2
\text{d6}+2 \text{d2} \text{d6})-11 (-\text{d3} \text{d5}+4 \text{d2} \text{d6})-3 (-\text{d1} \text{d2} \text{d5}+14 \text{d2} \text{d6}-5
(-\text{d1}^2 \text{d6}+2 \text{d2} \text{d6})-3 (-\text{d3} \text{d5}+4 \text{d2} \text{d6}))-4 (-\text{d4}^2+6 \text{d2}
\text{d6}-2 (-\text{d3} \text{d5}+4 \text{d2} \text{d6})))))+\text{c3}^3 (\text{d3}^3-93 \text{d3} \text{d6}+36 (-\text{d4}
\text{d5}+3 \text{d3} \text{d6})+36 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})+15 (-\text{d1} \text{d3} \text{d5}+15 \text{d3} \text{d6}-4
(-\text{d4} \text{d5}+3 \text{d3} \text{d6})-4 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6}))+6 (-\text{d2}^2 \text{d5}+24 \text{d3}
\text{d6}-6 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-9 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})-2 (-\text{d1} \text{d3} \text{d5}+15
\text{d3} \text{d6}-4 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-4 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})))+6 (-\text{d1}
\text{d4}^2+24 \text{d3} \text{d6}-9 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-6 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})-2 (-\text{d1}
\text{d3} \text{d5}+15 \text{d3} \text{d6}-4 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-4 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})))+3
(-\text{d2} \text{d3} \text{d4}+60 \text{d3} \text{d6}-22 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-22 (-\text{d1} \text{d2} \text{d6}+3
\text{d3} \text{d6})-8 (-\text{d1} \text{d3} \text{d5}+15 \text{d3} \text{d6}-4 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-4 (-\text{d1} \text{d2}
\text{d6}+3 \text{d3} \text{d6}))-3 (-\text{d2}^2 \text{d5}+24 \text{d3} \text{d6}-6 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-9 (-\text{d1}
\text{d2} \text{d6}+3 \text{d3} \text{d6})-2 (-\text{d1} \text{d3} \text{d5}+15 \text{d3} \text{d6}-4 (-\text{d4} \text{d5}+3 \text{d3} \text{d6})-4
(-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})))-3 (-\text{d1} \text{d4}^2+24 \text{d3} \text{d6}-9 (-\text{d4} \text{d5}+3 \text{d3}
\text{d6})-6 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})-2 (-\text{d1} \text{d3} \text{d5}+15 \text{d3} \text{d6}-4 (-\text{d4} \text{d5}+3
\text{d3} \text{d6})-4 (-\text{d1} \text{d2} \text{d6}+3 \text{d3} \text{d6})))))+\text{c2} \text{c3}^2 (\text{d3}^2 \text{d4}-80
\text{d4} \text{d6}+30 (-\text{d5}^2+2 \text{d4} \text{d6})+31 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6})+12 (-\text{d1}
\text{d4} \text{d5}+14 \text{d4} \text{d6}-5 (-\text{d5}^2+2 \text{d4} \text{d6})-3 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))+12
(-\text{d2}^2 \text{d6}+6 \text{d4} \text{d6}-2 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))+5 (-\text{d2} \text{d3} \text{d5}+32
\text{d4} \text{d6}-10 (-\text{d5}^2+2 \text{d4} \text{d6})-11 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6})-3 (-\text{d1}
\text{d4} \text{d5}+14 \text{d4} \text{d6}-5 (-\text{d5}^2+2 \text{d4} \text{d6})-3 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))-4
(-\text{d2}^2 \text{d6}+6 \text{d4} \text{d6}-2 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6})))+2 (-\text{d2} \text{d4}^2+53
\text{d4} \text{d6}-20 (-\text{d5}^2+2 \text{d4} \text{d6})-18 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6})-7 (-\text{d1}
\text{d4} \text{d5}+14 \text{d4} \text{d6}-5 (-\text{d5}^2+2 \text{d4} \text{d6})-3 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))-6
(-\text{d2}^2 \text{d6}+6 \text{d4} \text{d6}-2 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))-2 (-\text{d2} \text{d3} \text{d5}+32
\text{d4} \text{d6}-10 (-\text{d5}^2+2 \text{d4} \text{d6})-11 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6})-3 (-\text{d1}
\text{d4} \text{d5}+14 \text{d4} \text{d6}-5 (-\text{d5}^2+2 \text{d4} \text{d6})-3 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6}))-4
(-\text{d2}^2 \text{d6}+6 \text{d4} \text{d6}-2 (-\text{d1} \text{d3} \text{d6}+4 \text{d4} \text{d6})))))+\text{c1}
\text{c3}^2 (\text{d3} \text{d4}^2-80 \text{d5} \text{d6}+31 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6})+12 (-\text{d2} \text{d3}
\text{d6}+10 \text{d5} \text{d6}-3 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6}))+12 (-\text{d1} \text{d5}^2+11 \text{d5} \text{d6}-2
(-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6}))+5 (-\text{d2} \text{d4} \text{d5}+35 \text{d5} \text{d6}-11 (-\text{d1} \text{d4}
\text{d6}+5 \text{d5} \text{d6})-3 (-\text{d2} \text{d3} \text{d6}+10 \text{d5} \text{d6}-3 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6}))-4
(-\text{d1} \text{d5}^2+11 \text{d5} \text{d6}-2 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6})))+2 (-\text{d3}^2 \text{d5}+50
\text{d5} \text{d6}-18 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6})-7 (-\text{d2} \text{d3} \text{d6}+10 \text{d5} \text{d6}-3 (-\text{d1}
\text{d4} \text{d6}+5 \text{d5} \text{d6}))-6 (-\text{d1} \text{d5}^2+11 \text{d5} \text{d6}-2 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6}))-2
(-\text{d2} \text{d4} \text{d5}+35 \text{d5} \text{d6}-11 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6})-3 (-\text{d2} \text{d3} \text{d6}+10
\text{d5} \text{d6}-3 (-\text{d1} \text{d4} \text{d6}+5 \text{d5} \text{d6}))-4 (-\text{d1} \text{d5}^2+11 \text{d5} \text{d6}-2 (-\text{d1}
\text{d4} \text{d6}+5 \text{d5} \text{d6})))))+\text{c3}^2 (\text{d4}^3-90 \text{d6}^2+36 (-\text{d1} \text{d5}
\text{d6}+6 \text{d6}^2)+15 (-\text{d2} \text{d4} \text{d6}+15 \text{d6}^2-4 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2))+6
(-\text{d2} \text{d5}^2+30 \text{d6}^2-9 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)-2 (-\text{d2} \text{d4} \text{d6}+15
\text{d6}^2-4 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)))+6 (-\text{d3}^2 \text{d6}+20 \text{d6}^2-6 (-\text{d1}
\text{d5} \text{d6}+6 \text{d6}^2)-2 (-\text{d2} \text{d4} \text{d6}+15 \text{d6}^2-4 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)))+3
(-\text{d3} \text{d4} \text{d5}+60 \text{d6}^2-22 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)-8 (-\text{d2} \text{d4} \text{d6}+15
\text{d6}^2-4 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2))-3 (-\text{d2} \text{d5}^2+30 \text{d6}^2-9 (-\text{d1} \text{d5}
\text{d6}+6 \text{d6}^2)-2 (-\text{d2} \text{d4} \text{d6}+15 \text{d6}^2-4 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)))-3
(-\text{d3}^2 \text{d6}+20 \text{d6}^2-6 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)-2 (-\text{d2} \text{d4} \text{d6}+15
\text{d6}^2-4 (-\text{d1} \text{d5} \text{d6}+6 \text{d6}^2)))))\)
\end{doublespace}




==> chow_of_F_mathematica_2.tex <==
%% AMS-LaTeX Created with the Wolfram Language : www.wolfram.com


\begin{doublespace}
\noindent\(\pmb{\text{(*Define the Chern classes of the symmetric product*)}}\\
\pmb{}\\
\pmb{\text{S1}[\text{c1$\_$},\text{c2$\_$},\text{c3$\_$}]\text{:=}4 \text{c1};}\\
\pmb{\text{S2}[\text{c1$\_$},\text{c2$\_$},\text{c3$\_$}]\text{:=}5 \text{c1}{}^{\wedge}2+5 \text{c2};}\\
\pmb{\text{S3}[\text{c1$\_$},\text{c2$\_$},\text{c3$\_$}]\text{:=}2 \text{c1}{}^{\wedge}3+11 \text{c1} \text{c2}+7 \text{c3};}\\
\pmb{}\\
\pmb{\text{(*Define the Euler classes up to degree 3 in ci*)}}\\
\pmb{}\\
\pmb{\text{e1}=\text{d6}{}^{\wedge}3+\text{c1} \text{d5} \text{d6}{}^{\wedge}2+\text{c1}{}^{\wedge}2 \text{d4} \text{d6}{}^{\wedge}2+\text{c2} (\text{d5}{}^{\wedge}2
\text{d6}-2 \text{d4} \text{d6}{}^{\wedge}2)+\text{c1} \text{c2} (\text{d4} \text{d5} \text{d6}-3 \text{d3} \text{d6}{}^{\wedge}2)+}
\pmb{\text{c3} (\text{d5}{}^{\wedge}3-6 \text{d3} \text{d6}{}^{\wedge}2+3 (-\text{d4} \text{d5} \text{d6}+3 \text{d3} \text{d6}{}^{\wedge}2));}\\
\pmb{\text{e2}=(\text{C1}-\text{c1}){}^{\wedge}6+(\text{C1}-\text{c1}){}^{\wedge}5 \text{S1}[\text{c1},\text{c2},\text{c3}]+(\text{C1}-\text{c1}){}^{\wedge}4
\text{S2}[\text{c1},\text{c2},\text{c3}]+}\\
\pmb{(\text{C1}-\text{c1}){}^{\wedge}3 \text{S3}[\text{c1},\text{c2},\text{c3}];}\\
\pmb{\text{e3}=8 (\text{C1}-\text{c1}){}^{\wedge}3+4 (\text{C1}-\text{c1}){}^{\wedge}2 \text{c1}+2 (\text{C1}-\text{c1}) \text{c2}+\text{c3};}\\
\pmb{}\\
\pmb{\text{(*The class of } [\text{Tilde } F] \text{ up to degree } 3\text{*)}}\\
\pmb{}\\
\pmb{\text{final}=\text{e1} \text{e2} \text{e3};}\\
\pmb{\text{final}=\text{Expand}[\text{final}];}\\
\pmb{\text{Collect}[\text{final},\{\text{c1},\text{c2},\text{c3}\}]}\)
\end{doublespace}

\begin{doublespace}
\noindent\(8 \text{C1}^9 \text{d6}^3+\text{c3}^3 (7 \text{C1}^3 \text{d5}^3-21 \text{C1}^3 \text{d4} \text{d5} \text{d6}+21 \text{C1}^3 \text{d3}
\text{d6}^2)+\text{c2}^3 (10 \text{C1}^5 \text{d5}^2 \text{d6}-20 \text{C1}^5 \text{d4} \text{d6}^2)+\text{c1}^9 (4 \text{C1}^2
\text{d4} \text{d6}^2+24 \text{c2} \text{d4} \text{d6}^2)+\text{c3}^2 (57 \text{C1}^6 \text{d5}^3-171 \text{C1}^6 \text{d4} \text{d5}
\text{d6}+171 \text{C1}^6 \text{d3} \text{d6}^2+7 \text{C1}^3 \text{d6}^3)+\text{c3} (8 \text{C1}^9 \text{d5}^3-24 \text{C1}^9 \text{d4}
\text{d5} \text{d6}+24 \text{C1}^9 \text{d3} \text{d6}^2+57 \text{C1}^6 \text{d6}^3)+\text{c2}^2 (42 \text{C1}^7 \text{d5}^2 \text{d6}-84
\text{C1}^7 \text{d4} \text{d6}^2+10 \text{C1}^5 \text{d6}^3+\text{c3} (10 \text{C1}^5 \text{d5}^3-30 \text{C1}^5 \text{d4} \text{d5} \text{d6}+19
\text{C1}^4 \text{d5}^2 \text{d6}+30 \text{C1}^5 \text{d3} \text{d6}^2-38 \text{C1}^4 \text{d4} \text{d6}^2))+\text{c1}^8 (-24 \text{C1}^3
\text{d4} \text{d6}^2+28 \text{c3} \text{d4} \text{d6}^2+4 \text{C1}^2 \text{d5} \text{d6}^2+\text{c2}^2 (24 \text{d4} \text{d5} \text{d6}-72
\text{d3} \text{d6}^2)+\text{c2} (4 \text{C1}^2 \text{d4} \text{d5} \text{d6}-12 \text{C1}^2 \text{d3} \text{d6}^2-148 \text{C1} \text{d4}
\text{d6}^2+24 \text{d5} \text{d6}^2))+\text{c2} (8 \text{C1}^9 \text{d5}^2 \text{d6}-16 \text{C1}^9 \text{d4} \text{d6}^2+42 \text{C1}^7
\text{d6}^3+\text{c3}^2 (19 \text{C1}^4 \text{d5}^3-57 \text{C1}^4 \text{d4} \text{d5} \text{d6}+7 \text{C1}^3 \text{d5}^2 \text{d6}+57 \text{C1}^4
\text{d3} \text{d6}^2-14 \text{C1}^3 \text{d4} \text{d6}^2)+\text{c3} (42 \text{C1}^7 \text{d5}^3-126 \text{C1}^7 \text{d4} \text{d5}
\text{d6}+57 \text{C1}^6 \text{d5}^2 \text{d6}+126 \text{C1}^7 \text{d3} \text{d6}^2-114 \text{C1}^6 \text{d4} \text{d6}^2+19 \text{C1}^4 \text{d6}^3))+\text{c1}^7
(52 \text{C1}^4 \text{d4} \text{d6}^2-24 \text{C1}^3 \text{d5} \text{d6}^2+4 \text{C1}^2 \text{d6}^3+\text{c2}^2 (-148 \text{C1} \text{d4}
\text{d5} \text{d6}+24 \text{d5}^2 \text{d6}+444 \text{C1} \text{d3} \text{d6}^2-36 \text{d4} \text{d6}^2)+\text{c3} (4 \text{C1}^2 \text{d5}^3-12
\text{C1}^2 \text{d4} \text{d5} \text{d6}+12 \text{C1}^2 \text{d3} \text{d6}^2-196 \text{C1} \text{d4} \text{d6}^2+28 \text{d5} \text{d6}^2)+\text{c2}
(-24 \text{C1}^3 \text{d4} \text{d5} \text{d6}+4 \text{C1}^2 \text{d5}^2 \text{d6}+72 \text{C1}^3 \text{d3} \text{d6}^2+334 \text{C1}^2 \text{d4}
\text{d6}^2-148 \text{C1} \text{d5} \text{d6}^2+24 \text{d6}^3+\text{c3} (24 \text{d5}^3-44 \text{d4} \text{d5} \text{d6}-12 \text{d3} \text{d6}^2)))+\text{c1}^6
(-40 \text{C1}^5 \text{d4} \text{d6}^2+52 \text{C1}^4 \text{d5} \text{d6}^2-24 \text{C1}^3 \text{d6}^3+\text{c2}^3 (12 \text{d4} \text{d5}
\text{d6}-36 \text{d3} \text{d6}^2)+\text{c3}^2 (28 \text{d5}^3-84 \text{d4} \text{d5} \text{d6}+84 \text{d3} \text{d6}^2)+\text{c2}^2
(342 \text{C1}^2 \text{d4} \text{d5} \text{d6}-148 \text{C1} \text{d5}^2 \text{d6}-1026 \text{C1}^2 \text{d3} \text{d6}^2+258 \text{C1} \text{d4}
\text{d6}^2+12 \text{d5} \text{d6}^2)+\text{c3} (-24 \text{C1}^3 \text{d5}^3+72 \text{C1}^3 \text{d4} \text{d5} \text{d6}-72 \text{C1}^3
\text{d3} \text{d6}^2+559 \text{C1}^2 \text{d4} \text{d6}^2-196 \text{C1} \text{d5} \text{d6}^2+28 \text{d6}^3)+\text{c2} (52 \text{C1}^4
\text{d4} \text{d5} \text{d6}-24 \text{C1}^3 \text{d5}^2 \text{d6}-156 \text{C1}^4 \text{d3} \text{d6}^2-278 \text{C1}^3 \text{d4} \text{d6}^2+342
\text{C1}^2 \text{d5} \text{d6}^2-148 \text{C1} \text{d6}^3+\text{c3} (-148 \text{C1} \text{d5}^3+248 \text{C1} \text{d4} \text{d5} \text{d6}+28
\text{d5}^2 \text{d6}+144 \text{C1} \text{d3} \text{d6}^2-48 \text{d4} \text{d6}^2)))+\text{c1}^5 (-20 \text{C1}^6 \text{d4}
\text{d6}^2-40 \text{C1}^5 \text{d5} \text{d6}^2+52 \text{C1}^4 \text{d6}^3+\text{c2}^3 (-38 \text{C1} \text{d4} \text{d5} \text{d6}+12 \text{d5}^2
\text{d6}+114 \text{C1} \text{d3} \text{d6}^2-24 \text{d4} \text{d6}^2)+\text{c3}^2 (-196 \text{C1} \text{d5}^3+588 \text{C1} \text{d4}
\text{d5} \text{d6}-588 \text{C1} \text{d3} \text{d6}^2-7 \text{d4} \text{d6}^2)+\text{c3} (52 \text{C1}^4 \text{d5}^3-156 \text{C1}^4
\text{d4} \text{d5} \text{d6}+156 \text{C1}^4 \text{d3} \text{d6}^2-838 \text{C1}^3 \text{d4} \text{d6}^2+559 \text{C1}^2 \text{d5} \text{d6}^2-196
\text{C1} \text{d6}^3)+\text{c2}^2 (-326 \text{C1}^3 \text{d4} \text{d5} \text{d6}+342 \text{C1}^2 \text{d5}^2 \text{d6}+978 \text{C1}^3
\text{d3} \text{d6}^2-652 \text{C1}^2 \text{d4} \text{d6}^2-38 \text{C1} \text{d5} \text{d6}^2+12 \text{d6}^3+\text{c3} (12 \text{d5}^3-28 \text{d4}
\text{d5} \text{d6}+12 \text{d3} \text{d6}^2))+\text{c2} (-40 \text{C1}^5 \text{d4} \text{d5} \text{d6}+52 \text{C1}^4 \text{d5}^2
\text{d6}+120 \text{C1}^5 \text{d3} \text{d6}^2-100 \text{C1}^4 \text{d4} \text{d6}^2-326 \text{C1}^3 \text{d5} \text{d6}^2+342 \text{C1}^2 \text{d6}^3+\text{c3}
(342 \text{C1}^2 \text{d5}^3-467 \text{C1}^2 \text{d4} \text{d5} \text{d6}-196 \text{C1} \text{d5}^2 \text{d6}-651 \text{C1}^2 \text{d3} \text{d6}^2+349
\text{C1} \text{d4} \text{d6}^2+8 \text{d5} \text{d6}^2)))+\text{c1}^4 (56 \text{C1}^7 \text{d4} \text{d6}^2-20 \text{C1}^6
\text{d5} \text{d6}^2-40 \text{C1}^5 \text{d6}^3+\text{c2}^3 (32 \text{C1}^2 \text{d4} \text{d5} \text{d6}-38 \text{C1} \text{d5}^2 \text{d6}-96
\text{C1}^2 \text{d3} \text{d6}^2+76 \text{C1} \text{d4} \text{d6}^2)+\text{c3}^2 (559 \text{C1}^2 \text{d5}^3-1677 \text{C1}^2 \text{d4}
\text{d5} \text{d6}+1677 \text{C1}^2 \text{d3} \text{d6}^2+21 \text{C1} \text{d4} \text{d6}^2-7 \text{d5} \text{d6}^2)+\text{c3} (-40
\text{C1}^5 \text{d5}^3+120 \text{C1}^5 \text{d4} \text{d5} \text{d6}-120 \text{C1}^5 \text{d3} \text{d6}^2+700 \text{C1}^4 \text{d4} \text{d6}^2-838
\text{C1}^3 \text{d5} \text{d6}^2+559 \text{C1}^2 \text{d6}^3)+\text{c2}^2 (4 \text{C1}^4 \text{d4} \text{d5} \text{d6}-326 \text{C1}^3
\text{d5}^2 \text{d6}-12 \text{C1}^4 \text{d3} \text{d6}^2+664 \text{C1}^3 \text{d4} \text{d6}^2+32 \text{C1}^2 \text{d5} \text{d6}^2-38 \text{C1}
\text{d6}^3+\text{c3} (-38 \text{C1} \text{d5}^3+71 \text{C1} \text{d4} \text{d5} \text{d6}+8 \text{d5}^2 \text{d6}+15 \text{C1} \text{d3} \text{d6}^2-16
\text{d4} \text{d6}^2))+\text{c2} (-20 \text{C1}^6 \text{d4} \text{d5} \text{d6}-40 \text{C1}^5 \text{d5}^2 \text{d6}+60 \text{C1}^6
\text{d3} \text{d6}^2+320 \text{C1}^5 \text{d4} \text{d6}^2+4 \text{C1}^4 \text{d5} \text{d6}^2-326 \text{C1}^3 \text{d6}^3+\text{c3}^2 (8 \text{d5}^3-31
\text{d4} \text{d5} \text{d6}+45 \text{d3} \text{d6}^2)+\text{c3} (-326 \text{C1}^3 \text{d5}^3+140 \text{C1}^3 \text{d4} \text{d5} \text{d6}+559
\text{C1}^2 \text{d5}^2 \text{d6}+1536 \text{C1}^3 \text{d3} \text{d6}^2-1037 \text{C1}^2 \text{d4} \text{d6}^2-43 \text{C1} \text{d5} \text{d6}^2+8
\text{d6}^3)))+\text{c1}^3 (-36 \text{C1}^8 \text{d4} \text{d6}^2+56 \text{C1}^7 \text{d5} \text{d6}^2-20 \text{C1}^6 \text{d6}^3+\text{c3}^3
(-7 \text{d5}^3+21 \text{d4} \text{d5} \text{d6}-21 \text{d3} \text{d6}^2)+\text{c2}^3 (12 \text{C1}^3 \text{d4} \text{d5} \text{d6}+32
\text{C1}^2 \text{d5}^2 \text{d6}-36 \text{C1}^3 \text{d3} \text{d6}^2-64 \text{C1}^2 \text{d4} \text{d6}^2)+\text{c3}^2 (-838 \text{C1}^3
\text{d5}^3+2514 \text{C1}^3 \text{d4} \text{d5} \text{d6}-2514 \text{C1}^3 \text{d3} \text{d6}^2-21 \text{C1}^2 \text{d4} \text{d6}^2+21 \text{C1}
\text{d5} \text{d6}^2-7 \text{d6}^3)+\text{c3} (-20 \text{C1}^6 \text{d5}^3+60 \text{C1}^6 \text{d4} \text{d5} \text{d6}-60 \text{C1}^6
\text{d3} \text{d6}^2-310 \text{C1}^5 \text{d4} \text{d6}^2+700 \text{C1}^4 \text{d5} \text{d6}^2-838 \text{C1}^3 \text{d6}^3)+\text{c2}^2
(240 \text{C1}^5 \text{d4} \text{d5} \text{d6}+4 \text{C1}^4 \text{d5}^2 \text{d6}-720 \text{C1}^5 \text{d3} \text{d6}^2-36 \text{C1}^4 \text{d4}
\text{d6}^2+12 \text{C1}^3 \text{d5} \text{d6}^2+32 \text{C1}^2 \text{d6}^3+\text{c3} (32 \text{C1}^2 \text{d5}^3-15 \text{C1}^2 \text{d4} \text{d5}
\text{d6}-43 \text{C1} \text{d5}^2 \text{d6}-147 \text{C1}^2 \text{d3} \text{d6}^2+86 \text{C1} \text{d4} \text{d6}^2))+\text{c2} (56
\text{C1}^7 \text{d4} \text{d5} \text{d6}-20 \text{C1}^6 \text{d5}^2 \text{d6}-168 \text{C1}^7 \text{d3} \text{d6}^2-138 \text{C1}^6 \text{d4} \text{d6}^2+240
\text{C1}^5 \text{d5} \text{d6}^2+4 \text{C1}^4 \text{d6}^3+\text{c3}^2 (-43 \text{C1} \text{d5}^3+150 \text{C1} \text{d4} \text{d5} \text{d6}-7
\text{d5}^2 \text{d6}-192 \text{C1} \text{d3} \text{d6}^2+14 \text{d4} \text{d6}^2)+\text{c3} (4 \text{C1}^4 \text{d5}^3+688 \text{C1}^4
\text{d4} \text{d5} \text{d6}-838 \text{C1}^3 \text{d5}^2 \text{d6}-2088 \text{C1}^4 \text{d3} \text{d6}^2+1611 \text{C1}^3 \text{d4} \text{d6}^2+81
\text{C1}^2 \text{d5} \text{d6}^2-43 \text{C1} \text{d6}^3)))+\text{c1}^2 (8 \text{C1}^9 \text{d4} \text{d6}^2-36 \text{C1}^8
\text{d5} \text{d6}^2+56 \text{C1}^7 \text{d6}^3+\text{c3}^3 (21 \text{C1} \text{d5}^3-63 \text{C1} \text{d4} \text{d5} \text{d6}+63 \text{C1}
\text{d3} \text{d6}^2)+\text{c2}^3 (-28 \text{C1}^4 \text{d4} \text{d5} \text{d6}+12 \text{C1}^3 \text{d5}^2 \text{d6}+84 \text{C1}^4
\text{d3} \text{d6}^2-24 \text{C1}^3 \text{d4} \text{d6}^2)+\text{c3}^2 (700 \text{C1}^4 \text{d5}^3-2100 \text{C1}^4 \text{d4} \text{d5}
\text{d6}+2100 \text{C1}^4 \text{d3} \text{d6}^2+7 \text{C1}^3 \text{d4} \text{d6}^2-21 \text{C1}^2 \text{d5} \text{d6}^2+21 \text{C1} \text{d6}^3)+\text{c3}
(56 \text{C1}^7 \text{d5}^3-168 \text{C1}^7 \text{d4} \text{d5} \text{d6}+168 \text{C1}^7 \text{d3} \text{d6}^2+57 \text{C1}^6 \text{d4} \text{d6}^2-310
\text{C1}^5 \text{d5} \text{d6}^2+700 \text{C1}^4 \text{d6}^3)+\text{c2}^2 (-178 \text{C1}^6 \text{d4} \text{d5} \text{d6}+240 \text{C1}^5
\text{d5}^2 \text{d6}+534 \text{C1}^6 \text{d3} \text{d6}^2-470 \text{C1}^5 \text{d4} \text{d6}^2-28 \text{C1}^4 \text{d5} \text{d6}^2+12 \text{C1}^3
\text{d6}^3+\text{c3} (12 \text{C1}^3 \text{d5}^3-101 \text{C1}^3 \text{d4} \text{d5} \text{d6}+81 \text{C1}^2 \text{d5}^2 \text{d6}+231 \text{C1}^3
\text{d3} \text{d6}^2-162 \text{C1}^2 \text{d4} \text{d6}^2))+\text{c2} (-36 \text{C1}^8 \text{d4} \text{d5} \text{d6}+56 \text{C1}^7
\text{d5}^2 \text{d6}+108 \text{C1}^8 \text{d3} \text{d6}^2-70 \text{C1}^7 \text{d4} \text{d6}^2-178 \text{C1}^6 \text{d5} \text{d6}^2+240 \text{C1}^5
\text{d6}^3+\text{c3}^2 (81 \text{C1}^2 \text{d5}^3-264 \text{C1}^2 \text{d4} \text{d5} \text{d6}+21 \text{C1} \text{d5}^2 \text{d6}+306 \text{C1}^2
\text{d3} \text{d6}^2-42 \text{C1} \text{d4} \text{d6}^2)+\text{c3} (240 \text{C1}^5 \text{d5}^3-1030 \text{C1}^5 \text{d4} \text{d5}
\text{d6}+700 \text{C1}^4 \text{d5}^2 \text{d6}+1650 \text{C1}^5 \text{d3} \text{d6}^2-1381 \text{C1}^4 \text{d4} \text{d6}^2-65 \text{C1}^3 \text{d5}
\text{d6}^2+81 \text{C1}^2 \text{d6}^3)))+\text{c1} (8 \text{C1}^9 \text{d5} \text{d6}^2-36 \text{C1}^8 \text{d6}^3+\text{c3}^3
(-21 \text{C1}^2 \text{d5}^3+63 \text{C1}^2 \text{d4} \text{d5} \text{d6}-63 \text{C1}^2 \text{d3} \text{d6}^2)+\text{c2}^3 (10 \text{C1}^5
\text{d4} \text{d5} \text{d6}-28 \text{C1}^4 \text{d5}^2 \text{d6}-30 \text{C1}^5 \text{d3} \text{d6}^2+56 \text{C1}^4 \text{d4} \text{d6}^2)+\text{c3}^2
(-310 \text{C1}^5 \text{d5}^3+930 \text{C1}^5 \text{d4} \text{d5} \text{d6}-930 \text{C1}^5 \text{d3} \text{d6}^2+7 \text{C1}^3 \text{d5} \text{d6}^2-21
\text{C1}^2 \text{d6}^3)+\text{c3} (-36 \text{C1}^8 \text{d5}^3+108 \text{C1}^8 \text{d4} \text{d5} \text{d6}-108 \text{C1}^8 \text{d3}
\text{d6}^2+57 \text{C1}^6 \text{d5} \text{d6}^2-310 \text{C1}^5 \text{d6}^3)+\text{c2}^2 (42 \text{C1}^7 \text{d4} \text{d5} \text{d6}-178
\text{C1}^6 \text{d5}^2 \text{d6}-126 \text{C1}^7 \text{d3} \text{d6}^2+356 \text{C1}^6 \text{d4} \text{d6}^2+10 \text{C1}^5 \text{d5} \text{d6}^2-28
\text{C1}^4 \text{d6}^3+\text{c3} (-28 \text{C1}^4 \text{d5}^3+103 \text{C1}^4 \text{d4} \text{d5} \text{d6}-65 \text{C1}^3 \text{d5}^2 \text{d6}-141
\text{C1}^4 \text{d3} \text{d6}^2+130 \text{C1}^3 \text{d4} \text{d6}^2))+\text{c2} (8 \text{C1}^9 \text{d4} \text{d5} \text{d6}-36
\text{C1}^8 \text{d5}^2 \text{d6}-24 \text{C1}^9 \text{d3} \text{d6}^2+72 \text{C1}^8 \text{d4} \text{d6}^2+42 \text{C1}^7 \text{d5} \text{d6}^2-178
\text{C1}^6 \text{d6}^3+\text{c3}^2 (-65 \text{C1}^3 \text{d5}^3+202 \text{C1}^3 \text{d4} \text{d5} \text{d6}-21 \text{C1}^2 \text{d5}^2 \text{d6}-216
\text{C1}^3 \text{d3} \text{d6}^2+42 \text{C1}^2 \text{d4} \text{d6}^2)+\text{c3} (-178 \text{C1}^6 \text{d5}^3+591 \text{C1}^6 \text{d4}
\text{d5} \text{d6}-310 \text{C1}^5 \text{d5}^2 \text{d6}-705 \text{C1}^6 \text{d3} \text{d6}^2+620 \text{C1}^5 \text{d4} \text{d6}^2+19 \text{C1}^4
\text{d5} \text{d6}^2-65 \text{C1}^3 \text{d6}^3)))\)
\end{doublespace}




==> chow_of_F_sage.tex <==

    

    
    
    % Colors for the hyperref package
    \definecolor{urlcolor}{rgb}{0,.145,.698}
    \definecolor{linkcolor}{rgb}{.71,0.21,0.01}
    \definecolor{citecolor}{rgb}{.12,.54,.11}

    % ANSI colors
    \definecolor{ansi-black}{HTML}{3E424D}
    \definecolor{ansi-black-intense}{HTML}{282C36}
    \definecolor{ansi-red}{HTML}{E75C58}
    \definecolor{ansi-red-intense}{HTML}{B22B31}
    \definecolor{ansi-green}{HTML}{00A250}
    \definecolor{ansi-green-intense}{HTML}{007427}
    \definecolor{ansi-yellow}{HTML}{DDB62B}
    \definecolor{ansi-yellow-intense}{HTML}{B27D12}
    \definecolor{ansi-blue}{HTML}{208FFB}
    \definecolor{ansi-blue-intense}{HTML}{0065CA}
    \definecolor{ansi-magenta}{HTML}{D160C4}
    \definecolor{ansi-magenta-intense}{HTML}{A03196}
    \definecolor{ansi-cyan}{HTML}{60C6C8}
    \definecolor{ansi-cyan-intense}{HTML}{258F8F}
    \definecolor{ansi-white}{HTML}{C5C1B4}
    \definecolor{ansi-white-intense}{HTML}{A1A6B2}
    \definecolor{ansi-default-inverse-fg}{HTML}{FFFFFF}
    \definecolor{ansi-default-inverse-bg}{HTML}{000000}

    % commands and environments needed by pandoc snippets
    % extracted from the output of `pandoc -s`
    \providecommand{\tightlist}{%
      \setlength{\itemsep}{0pt}\setlength{\parskip}{0pt}}
    \DefineVerbatimEnvironment{Highlighting}{Verbatim}{commandchars=\\\{\}}
    % Add ',fontsize=\small' for more characters per line
    \newenvironment{Shaded}{}{}
    \newcommand{\KeywordTok}[1]{\textcolor[rgb]{0.00,0.44,0.13}{\textbf{{#1}}}}
    \newcommand{\DataTypeTok}[1]{\textcolor[rgb]{0.56,0.13,0.00}{{#1}}}
    \newcommand{\DecValTok}[1]{\textcolor[rgb]{0.25,0.63,0.44}{{#1}}}
    \newcommand{\BaseNTok}[1]{\textcolor[rgb]{0.25,0.63,0.44}{{#1}}}
    \newcommand{\FloatTok}[1]{\textcolor[rgb]{0.25,0.63,0.44}{{#1}}}
    \newcommand{\CharTok}[1]{\textcolor[rgb]{0.25,0.44,0.63}{{#1}}}
    \newcommand{\StringTok}[1]{\textcolor[rgb]{0.25,0.44,0.63}{{#1}}}
    \newcommand{\CommentTok}[1]{\textcolor[rgb]{0.38,0.63,0.69}{\textit{{#1}}}}
    \newcommand{\OtherTok}[1]{\textcolor[rgb]{0.00,0.44,0.13}{{#1}}}
    \newcommand{\AlertTok}[1]{\textcolor[rgb]{1.00,0.00,0.00}{\textbf{{#1}}}}
    \newcommand{\FunctionTok}[1]{\textcolor[rgb]{0.02,0.16,0.49}{{#1}}}
    \newcommand{\RegionMarkerTok}[1]{{#1}}
    \newcommand{\ErrorTok}[1]{\textcolor[rgb]{1.00,0.00,0.00}{\textbf{{#1}}}}
    \newcommand{\NormalTok}[1]{{#1}}
    
    % Additional commands for more recent versions of Pandoc
    \newcommand{\ConstantTok}[1]{\textcolor[rgb]{0.53,0.00,0.00}{{#1}}}
    \newcommand{\SpecialCharTok}[1]{\textcolor[rgb]{0.25,0.44,0.63}{{#1}}}
    \newcommand{\VerbatimStringTok}[1]{\textcolor[rgb]{0.25,0.44,0.63}{{#1}}}
    \newcommand{\SpecialStringTok}[1]{\textcolor[rgb]{0.73,0.40,0.53}{{#1}}}
    \newcommand{\ImportTok}[1]{{#1}}
    \newcommand{\DocumentationTok}[1]{\textcolor[rgb]{0.73,0.13,0.13}{\textit{{#1}}}}
    \newcommand{\AnnotationTok}[1]{\textcolor[rgb]{0.38,0.63,0.69}{\textbf{\textit{{#1}}}}}
    \newcommand{\CommentVarTok}[1]{\textcolor[rgb]{0.38,0.63,0.69}{\textbf{\textit{{#1}}}}}
    \newcommand{\VariableTok}[1]{\textcolor[rgb]{0.10,0.09,0.49}{{#1}}}
    \newcommand{\ControlFlowTok}[1]{\textcolor[rgb]{0.00,0.44,0.13}{\textbf{{#1}}}}
    \newcommand{\OperatorTok}[1]{\textcolor[rgb]{0.40,0.40,0.40}{{#1}}}
    \newcommand{\BuiltInTok}[1]{{#1}}
    \newcommand{\ExtensionTok}[1]{{#1}}
    \newcommand{\PreprocessorTok}[1]{\textcolor[rgb]{0.74,0.48,0.00}{{#1}}}
    \newcommand{\AttributeTok}[1]{\textcolor[rgb]{0.49,0.56,0.16}{{#1}}}
    \newcommand{\InformationTok}[1]{\textcolor[rgb]{0.38,0.63,0.69}{\textbf{\textit{{#1}}}}}
    \newcommand{\WarningTok}[1]{\textcolor[rgb]{0.38,0.63,0.69}{\textbf{\textit{{#1}}}}}
    
    
    % Define a nice break command that doesn't care if a line doesn't already
    % exist.
    \def\br{\hspace*{\fill} \\* }
    % Math Jax compatibility definitions
    \def\gt{>}
    \def\lt{<}
    \let\Oldtex\TeX
    \let\Oldlatex\LaTeX
    \renewcommand{\TeX}{\textrm{\Oldtex}}
    \renewcommand{\LaTeX}{\textrm{\Oldlatex}}
    % Document parameters
    % Document title
    
    
    
    
    
    

    % Pygments definitions
    
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother


    % Exact colors from NB
    \definecolor{incolor}{rgb}{0.0, 0.0, 0.5}
    \definecolor{outcolor}{rgb}{0.545, 0.0, 0.0}



    
    % Prevent overflowing lines due to hard-to-break entities
    \sloppy 
    % Setup hyperref package
    \hypersetup{
      breaklinks=true,  % so long urls are correctly broken across lines
      colorlinks=true,
      urlcolor=urlcolor,
      linkcolor=linkcolor,
      citecolor=citecolor,
      }
    % Slightly bigger margins than the latex defaults

    
    

  
    
    

    
    \begin{Verbatim}[commandchars=\\\{\}]
{\color{incolor}In [{\color{incolor}1}
]:} \PY{c+c1}{\PYZsh{} Define the Schur\PYZsq{}s polynomials}
        \PY{n}{R} \PY{o}{=} \PY{n}{SymmetricFunctions}\PY{p}{(}\PY{n}{QQ}\PY{p}{)}
        \PY{n}{s} \PY{o}{=} \PY{n}{R}\PY{o}{.}\PY{n}{schur}\PY{p}{(}\PY{p}{)}
        
        \PY{c+c1}{\PYZsh{}The expressions of the coefficients}
        \PY{n}{coef\PYZus{}of\PYZus{}c1c1c1} \PY{o}{=} \PY{o}{\PYZhy{}}\PY{l+m+mi}{36} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{8} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{4}\PY{p}{]} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{2} \PY{o}{+} \PYZbs{}
            \PY{l+m+mi}{56} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{7} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{5}\PY{p}{]} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{2} \PY{o}{\PYZhy{}} \PY{l+m+mi}{20} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{6} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{3}
        \PY{n}{coef\PYZus{}of\PYZus{}c1c2} \PY{o}{=} \PY{l+m+mi}{8} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{9} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{4}\PY{p}{]} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{5}\PY{p}{]} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]} \PY{o}{\PYZhy{}} \PYZbs{}
            \PY{l+m+mi}{36} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{8} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{5}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{2} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]} \PY{o}{\PYZhy{}} \PY{l+m+mi}{24} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{9} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{3}\PY{p}{]} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{2} \PY{o}{+} \PYZbs{}
            \PY{l+m+mi}{72} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{8} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{4}\PY{p}{]} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{2} \PY{o}{+} \PY{l+m+mi}{42} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{7} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{5}\PY{p}{]} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{2} \PY{o}{\PYZhy{}} \PYZbs{}
            \PY{l+m+mi}{178} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{6} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{3}
        \PY{n}{coef\PYZus{}of\PYZus{}c3} \PY{o}{=} \PY{l+m+mi}{8} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{9} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{5}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{3} \PY{o}{\PYZhy{}} \PYZbs{}
            \PY{l+m+mi}{24} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{9} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{4}\PY{p}{]} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{5}\PY{p}{]} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]} \PY{o}{+} \PYZbs{}
            \PY{l+m+mi}{24} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{9} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{3}\PY{p}{]} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{2} \PY{o}{+} \PY{l+m+mi}{57} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{6} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{]}\PY{o}{\PYZca{}}\PY{l+m+mi}{3}
            
        \PY{c+c1}{\PYZsh{}Define a function that finds the coefficient of s[6,6,6,6]}
        \PY{k}{def} \PY{n+nf}{find\PYZus{}num}\PY{p}{(}\PY{n}{expr}\PY{p}{)}\PY{p}{:}
            \PY{k}{for} \PY{n}{part} \PY{o+ow}{in} \PY{n}{expr}\PY{p}{:}
                \PY{k}{if} \PY{n}{part}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{o}{==}\PY{p}{[}\PY{l+m+mi}{6}\PY{p}{,}\PY{l+m+mi}{6}\PY{p}{,}\PY{l+m+mi}{6}\PY{p}{,}\PY{l+m+mi}{6}\PY{p}{]}\PY{p}{:}
                    \PY{k}{return} \PY{n}{part}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}
        
        \PY{c+c1}{\PYZsh{}Print the final result}
        \PY{n+nb}{print}\PY{p}{(}
            \PY{n}{f}\PY{l+s+s1}{\PYZsq{}}\PY{l+s+s1}{The expression of [F] is (}\PY{l+s+s1}{\PYZob{}}\PY{l+s+s1}{find\PYZus{}num(coef\PYZus{}of\PYZus{}c1c1c1)\PYZcb{}).c1\PYZca{}3 }\PY{l+s+se}{\PYZbs{}}
        \PY{l+s+s1}{+ (}\PY{l+s+s1}{\PYZob{}}\PY{l+s+s1}{find\PYZus{}num(coef\PYZus{}of\PYZus{}c1c2)\PYZcb{}).c1c2 + (}\PY{l+s+s1}{\PYZob{}}\PY{l+s+s1}{find\PYZus{}num(coef\PYZus{}of\PYZus{}c3)\PYZcb{}).c3.}\PY{l+s+s1}{\PYZsq{}}
        \PY{p}{)}
\end{Verbatim}

    \begin{Verbatim}[commandchars=\\\{\}]
The expression of [F] is (-404).c1\^{}3 + (110).c1c2 + (49).c3.

    \end{Verbatim}


    % Add a bibliography block to the postdoc
    
    
    



==> hodge_numbers_sage.tex <==
% Colors for the hyperref package
    \definecolor{urlcolor}{rgb}{0,.145,.698}
    \definecolor{linkcolor}{rgb}{.71,0.21,0.01}
    \definecolor{citecolor}{rgb}{.12,.54,.11}

    % ANSI colors
    \definecolor{ansi-black}{HTML}{3E424D}
    \definecolor{ansi-black-intense}{HTML}{282C36}
    \definecolor{ansi-red}{HTML}{E75C58}
    \definecolor{ansi-red-intense}{HTML}{B22B31}
    \definecolor{ansi-green}{HTML}{00A250}
    \definecolor{ansi-green-intense}{HTML}{007427}
    \definecolor{ansi-yellow}{HTML}{DDB62B}
    \definecolor{ansi-yellow-intense}{HTML}{B27D12}
    \definecolor{ansi-blue}{HTML}{208FFB}
    \definecolor{ansi-blue-intense}{HTML}{0065CA}
    \definecolor{ansi-magenta}{HTML}{D160C4}
    \definecolor{ansi-magenta-intense}{HTML}{A03196}
    \definecolor{ansi-cyan}{HTML}{60C6C8}
    \definecolor{ansi-cyan-intense}{HTML}{258F8F}
    \definecolor{ansi-white}{HTML}{C5C1B4}
    \definecolor{ansi-white-intense}{HTML}{A1A6B2}
    \definecolor{ansi-default-inverse-fg}{HTML}{FFFFFF}
    \definecolor{ansi-default-inverse-bg}{HTML}{000000}

    % commands and environments needed by pandoc snippets
    % extracted from the output of `pandoc -s`
    \providecommand{\tightlist}{%
      \setlength{\itemsep}{0pt}\setlength{\parskip}{0pt}}
    \DefineVerbatimEnvironment{Highlighting}{Verbatim}{commandchars=\\\{\}}
    % Add ',fontsize=\small' for more characters per line
   
    
    % Define a nice break command that doesn't care if a line doesn't already
    % exist.
    \def\br{\hspace*{\fill} \\* }
    % Math Jax compatibility definitions
    \def\gt{>}
    \def\lt{<}
    \let\Oldtex\TeX
    \let\Oldlatex\LaTeX
    \renewcommand{\TeX}{\textrm{\Oldtex}}
    \renewcommand{\LaTeX}{\textrm{\Oldlatex}}
    % Document parameters
    % Document title
   
    
    
    
    
    

    % Pygments definitions
    
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother


    % Exact colors from NB
    \definecolor{incolor}{rgb}{0.0, 0.0, 0.5}
    \definecolor{outcolor}{rgb}{0.545, 0.0, 0.0}



    
    % Prevent overflowing lines due to hard-to-break entities
    \sloppy 
    % Setup hyperref package
    \hypersetup{
      breaklinks=true,  % so long urls are correctly broken across lines
      colorlinks=true,
      urlcolor=urlcolor,
      linkcolor=linkcolor,
      citecolor=citecolor,
      }
    % Slightly bigger margins than the latex defaults
    
    
    

  
    
    
    
    
    

    
    \begin{Verbatim}[commandchars=\\\{\}]
{\color{incolor}In [{\color{incolor}1}]:} \PY{n}{R} \PY{o}{=} \PY{n}{SymmetricFunctions}\PY{p}{(}\PY{n}{QQ}\PY{p}{)}
        \PY{n}{s} \PY{o}{=} \PY{n}{R}\PY{o}{.}\PY{n}{schur}\PY{p}{(}\PY{p}{)}
\end{Verbatim}

    \begin{Verbatim}[commandchars=\\\{\}]
{\color{incolor}In [{\color{incolor}2}]:} \PY{k}{def} \PY{n+nf}{mergeSortAndCount}\PY{p}{(}\PY{n}{arr}\PY{p}{,} \PY{n}{temp\PYZus{}arr}\PY{p}{,} \PY{n}{left}\PY{p}{,} \PY{n}{right}\PY{p}{)}\PY{p}{:}
            \PY{c+c1}{\PYZsh{} Initialize the inversion count}
            \PY{n}{inv\PYZus{}count} \PY{o}{=} \PY{l+m+mi}{0}
        
            \PY{c+c1}{\PYZsh{} If the list is not yet of length one}
            \PY{k}{if} \PY{n}{left} \PY{o}{\PYZlt{}} \PY{n}{right}\PY{p}{:}
                \PY{c+c1}{\PYZsh{} Mid is the point where the array is divided into two subarrays}
                \PY{n}{mid} \PY{o}{=} \PY{p}{(}\PY{n}{left} \PY{o}{+} \PY{n}{right}\PY{p}{)} \PY{o}{/}\PY{o}{/} \PY{l+m+mi}{2}
        
                \PY{c+c1}{\PYZsh{} Inversion count will be the sum of inversions in left\PYZhy{}part, \PYZbs{}}
                \PY{c+c1}{\PYZsh{} right\PYZhy{}part and number of inversions in merging}
                \PY{n}{inv\PYZus{}count} \PY{o}{+}\PY{o}{=} \PY{n}{mergeSortAndCount}\PY{p}{(}\PY{n}{arr}\PY{p}{,} \PY{n}{temp\PYZus{}arr}\PY{p}{,} \PY{n}{left}\PY{p}{,} \PY{n}{mid}\PY{p}{)}
                \PY{n}{inv\PYZus{}count} \PY{o}{+}\PY{o}{=} \PY{n}{mergeSortAndCount}\PY{p}{(}\PY{n}{arr}\PY{p}{,} \PY{n}{temp\PYZus{}arr}\PY{p}{,} \PY{n}{mid} \PY{o}{+} \PY{l+m+mi}{1}\PY{p}{,} \PY{n}{right}\PY{p}{)}
        
                \PY{c+c1}{\PYZsh{} Merging the two parts}
                \PY{n}{inv\PYZus{}count} \PY{o}{+}\PY{o}{=} \PY{n}{merge}\PY{p}{(}\PY{n}{arr}\PY{p}{,} \PY{n}{temp\PYZus{}arr}\PY{p}{,} \PY{n}{left}\PY{p}{,} \PY{n}{mid}\PY{p}{,} \PY{n}{right}\PY{p}{)}
        
            \PY{k}{return} \PY{n}{inv\PYZus{}count}
        
        \PY{k}{def} \PY{n+nf}{merge}\PY{p}{(}\PY{n}{arr}\PY{p}{,} \PY{n}{temp\PYZus{}arr}\PY{p}{,} \PY{n}{left}\PY{p}{,} \PY{n}{mid}\PY{p}{,} \PY{n}{right}\PY{p}{)}\PY{p}{:}
            \PY{n}{i} \PY{o}{=} \PY{n}{left}     \PY{c+c1}{\PYZsh{} Starting index of left subarray}
            \PY{n}{j} \PY{o}{=} \PY{n}{mid} \PY{o}{+} \PY{l+m+mi}{1}  \PY{c+c1}{\PYZsh{} Starting index of right subarray}
            \PY{n}{k} \PY{o}{=} \PY{n}{left}     \PY{c+c1}{\PYZsh{} Starting index of to be sorted subarray}
            \PY{n}{inv\PYZus{}count} \PY{o}{=} \PY{l+m+mi}{0}
        
            \PY{c+c1}{\PYZsh{} Conditions are checked to make sure that i and j don\PYZsq{}t \PYZbs{}}
            \PY{c+c1}{\PYZsh{} exceed their subarray limits}
            \PY{k}{while} \PY{n}{i} \PY{o}{\PYZlt{}}\PY{o}{=} \PY{n}{mid} \PY{o+ow}{and} \PY{n}{j} \PY{o}{\PYZlt{}}\PY{o}{=} \PY{n}{right}\PY{p}{:}
                \PY{c+c1}{\PYZsh{} There will be no inversion if arr[i] \PYZlt{}= arr[j]}
                \PY{k}{if} \PY{n}{arr}\PY{p}{[}\PY{n}{i}\PY{p}{]} \PY{o}{\PYZlt{}}\PY{o}{=} \PY{n}{arr}\PY{p}{[}\PY{n}{j}\PY{p}{]}\PY{p}{:}
                    \PY{n}{temp\PYZus{}arr}\PY{p}{[}\PY{n}{k}\PY{p}{]} \PY{o}{=} \PY{n}{arr}\PY{p}{[}\PY{n}{i}\PY{p}{]}
                    \PY{n}{k} \PY{o}{+}\PY{o}{=} \PY{l+m+mi}{1}
                    \PY{n}{i} \PY{o}{+}\PY{o}{=} \PY{l+m+mi}{1}
                \PY{k}{else}\PY{p}{:}
                    \PY{c+c1}{\PYZsh{} Inversion will occur}
                    \PY{n}{temp\PYZus{}arr}\PY{p}{[}\PY{n}{k}\PY{p}{]} \PY{o}{=} \PY{n}{arr}\PY{p}{[}\PY{n}{j}\PY{p}{]}
                    \PY{n}{inv\PYZus{}count} \PY{o}{+}\PY{o}{=} \PY{p}{(}\PY{n}{mid} \PY{o}{\PYZhy{}} \PY{n}{i} \PY{o}{+} \PY{l+m+mi}{1}\PY{p}{)}  \PY{c+c1}{\PYZsh{} Count the inversions}
                    \PY{n}{k} \PY{o}{+}\PY{o}{=} \PY{l+m+mi}{1}
                    \PY{n}{j} \PY{o}{+}\PY{o}{=} \PY{l+m+mi}{1}
        
            \PY{c+c1}{\PYZsh{} Copy the remaining elements of left subarray into temporary array}
            \PY{k}{while} \PY{n}{i} \PY{o}{\PYZlt{}}\PY{o}{=} \PY{n}{mid}\PY{p}{:}
                \PY{n}{temp\PYZus{}arr}\PY{p}{[}\PY{n}{k}\PY{p}{]} \PY{o}{=} \PY{n}{arr}\PY{p}{[}\PY{n}{i}\PY{p}{]}
                \PY{n}{k} \PY{o}{+}\PY{o}{=} \PY{l+m+mi}{1}
                \PY{n}{i} \PY{o}{+}\PY{o}{=} \PY{l+m+mi}{1}
        
            \PY{c+c1}{\PYZsh{} Copy the remaining elements of right subarray into temporary array}
            \PY{k}{while} \PY{n}{j} \PY{o}{\PYZlt{}}\PY{o}{=} \PY{n}{right}\PY{p}{:}
                \PY{n}{temp\PYZus{}arr}\PY{p}{[}\PY{n}{k}\PY{p}{]} \PY{o}{=} \PY{n}{arr}\PY{p}{[}\PY{n}{j}\PY{p}{]}
                \PY{n}{k} \PY{o}{+}\PY{o}{=} \PY{l+m+mi}{1}
                \PY{n}{j} \PY{o}{+}\PY{o}{=} \PY{l+m+mi}{1}
        
            \PY{c+c1}{\PYZsh{} Copy the sorted subarray into Original array}
            \PY{k}{for} \PY{n}{loop\PYZus{}var} \PY{o+ow}{in} \PY{n+nb}{range}\PY{p}{(}\PY{n}{left}\PY{p}{,} \PY{n}{right} \PY{o}{+} \PY{l+m+mi}{1}\PY{p}{)}\PY{p}{:}
                \PY{n}{arr}\PY{p}{[}\PY{n}{loop\PYZus{}var}\PY{p}{]} \PY{o}{=} \PY{n}{temp\PYZus{}arr}\PY{p}{[}\PY{n}{loop\PYZus{}var}\PY{p}{]}
        
            \PY{k}{return} \PY{n}{inv\PYZus{}count}
        
        \PY{k}{def} \PY{n+nf}{inversionCount}\PY{p}{(}\PY{n}{arr}\PY{p}{)}\PY{p}{:}
            \PY{c+c1}{\PYZsh{} Temporary array to be used in merge function}
            \PY{n}{temp\PYZus{}arr} \PY{o}{=} \PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{o}{*}\PY{n+nb}{len}\PY{p}{(}\PY{n}{arr}\PY{p}{)}
            \PY{k}{return} \PY{n}{mergeSortAndCount}\PY{p}{(}\PY{n}{arr}\PY{p}{,} \PY{n}{temp\PYZus{}arr}\PY{p}{,} \PY{l+m+mi}{0}\PY{p}{,} \PY{n+nb}{len}\PY{p}{(}\PY{n}{arr}\PY{p}{)} \PY{o}{\PYZhy{}} \PY{l+m+mi}{1}\PY{p}{)}
\end{Verbatim}

    \begin{Verbatim}[commandchars=\\\{\}]
{\color{incolor}In [{\color{incolor}3}]:} \PY{k}{def} \PY{n+nf}{dimension}\PY{p}{(}\PY{n}{w}\PY{p}{,} \PY{n}{n}\PY{p}{)}\PY{p}{:}
            \PY{c+c1}{\PYZsh{} The dimension of the representation L\PYZus{}wV\PYZus{}n.}
        
            \PY{n}{R}\PY{o}{=}\PY{n}{SymmetricFunctions}\PY{p}{(}\PY{n}{QQ}\PY{p}{)}
            \PY{k}{if} \PY{n}{w}\PY{p}{[}\PY{o}{\PYZhy{}}\PY{l+m+mi}{1}\PY{p}{]} \PY{o}{\PYZlt{}} \PY{l+m+mi}{0}\PY{p}{:}
                \PY{n}{w} \PY{o}{=} \PY{p}{[}\PY{o}{\PYZhy{}}\PY{n}{w}\PY{p}{[}\PY{o}{\PYZhy{}}\PY{n}{i}\PY{p}{]} \PY{k}{for} \PY{n}{i} \PY{o+ow}{in} \PY{n+nb}{range}\PY{p}{(}\PY{l+m+mi}{1}\PY{p}{,} \PY{n+nb}{len}\PY{p}{(}\PY{n}{w}\PY{p}{)}\PY{o}{+}\PY{l+m+mi}{1}\PY{p}{)}\PY{p}{]}
            \PY{k}{return} \PY{n+nb}{sum}\PY{p}{(}\PY{n}{s}\PY{p}{[}\PY{n}{w}\PY{p}{]}\PY{o}{.}\PY{n}{expand}\PY{p}{(}\PY{n}{n}\PY{p}{)}\PY{o}{.}\PY{n}{coefficients}\PY{p}{(}\PY{p}{)}\PY{p}{)}
            
\end{Verbatim}

    \begin{Verbatim}[commandchars=\\\{\}]
{\color{incolor}In [{\color{incolor}4}]:} \PY{k}{def} \PY{n+nf}{calculate\PYZus{}cohomology}\PY{p}{(}\PY{n}{schur\PYZus{}e}\PY{p}{,} \PY{n}{schur\PYZus{}q}\PY{p}{,} \PY{n}{r}\PY{p}{,} \PY{n}{n}\PY{p}{)}\PY{p}{:}
             
             \PY{l+s+sd}{\PYZdq{}\PYZdq{}\PYZdq{}}
         \PY{l+s+sd}{    Given:}
         \PY{l+s+sd}{        the Schur weights of the tautological sub and quotient \PYZbs{}}
         \PY{l+s+sd}{        bundles over the Grassmannian Gr(r, n),}
         \PY{l+s+sd}{    return:}
         \PY{l+s+sd}{        None in the irregular case;}
         \PY{l+s+sd}{        the index and the dimension of the cohomology in the \PYZbs{}}
         \PY{l+s+sd}{        regualar case.}
         \PY{l+s+sd}{    \PYZdq{}\PYZdq{}\PYZdq{}}
         
             \PY{c+c1}{\PYZsh{} Extend schur\PYZus{}e and schur\PYZus{}q lists with zeros}
             \PY{n}{schur\PYZus{}e} \PY{o}{+}\PY{o}{=} \PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]} \PY{o}{*} \PY{p}{(}\PY{n}{r} \PY{o}{\PYZhy{}} \PY{n+nb}{len}\PY{p}{(}\PY{n}{schur\PYZus{}e}\PY{p}{)}\PY{p}{)}
             \PY{n}{schur\PYZus{}q} \PY{o}{+}\PY{o}{=} \PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]} \PY{o}{*} \PY{p}{(}\PY{n}{n} \PY{o}{\PYZhy{}} \PY{n}{r} \PY{o}{\PYZhy{}} \PY{n+nb}{len}\PY{p}{(}\PY{n}{schur\PYZus{}q}\PY{p}{)}\PY{p}{)}
             
             \PY{c+c1}{\PYZsh{} Concatenate schur\PYZus{}e and schur\PYZus{}q}
             \PY{n}{schur} \PY{o}{=} \PY{n}{schur\PYZus{}q} \PY{o}{+} \PY{n}{schur\PYZus{}e}
             
             \PY{c+c1}{\PYZsh{} Generate delta list}
             \PY{n}{delta} \PY{o}{=} \PY{p}{[}\PY{n}{i} \PY{k}{for} \PY{n}{i} \PY{o+ow}{in} \PY{n+nb}{range}\PY{p}{(}\PY{l+m+mi}{1}\PY{p}{,} \PY{n}{n}\PY{o}{+}\PY{l+m+mi}{1}\PY{p}{)}\PY{p}{]}
             
            
             
             \PY{c+c1}{\PYZsh{} Calculate N}
             \PY{n}{N} \PY{o}{=} \PY{n}{r} \PY{o}{*} \PY{p}{(}\PY{n}{n} \PY{o}{\PYZhy{}} \PY{n}{r}\PY{p}{)}
             
             
             \PY{c+c1}{\PYZsh{} Element\PYZhy{}wise subtraction of delta from schur}
             \PY{n}{schur\PYZus{}delta} \PY{o}{=} \PY{p}{[}\PY{n}{s} \PY{o}{\PYZhy{}} \PY{n}{d} \PY{k}{for} \PY{n}{s}\PY{p}{,} \PY{n}{d} \PY{o+ow}{in} \PY{n+nb}{zip}\PY{p}{(}\PY{n}{schur}\PY{p}{,} \PY{n}{delta}\PY{p}{)}\PY{p}{]}
         
             \PY{c+c1}{\PYZsh{} Check for no duplicates and non\PYZhy{}negative values}
             \PY{k}{if} \PY{n+nb}{len}\PY{p}{(}\PY{n}{schur\PYZus{}delta}\PY{p}{)} \PY{o}{==} \PY{n+nb}{len}\PY{p}{(}\PY{n+nb}{set}\PY{p}{(}\PY{n}{schur\PYZus{}delta}\PY{p}{)}\PY{p}{)}\PY{p}{:}
                 \PY{n}{ind} \PY{o}{=} \PY{n}{inversionCount}\PY{p}{(}\PY{n}{schur\PYZus{}delta}\PY{p}{[}\PY{p}{:}\PY{p}{:}\PY{o}{\PYZhy{}}\PY{l+m+mi}{1}\PY{p}{]}\PY{p}{)}
                 \PY{n}{schur\PYZus{}delta\PYZus{}sorted} \PY{o}{=} \PY{n+nb}{sorted}\PY{p}{(}\PY{n}{schur\PYZus{}delta}\PY{p}{,} \PY{n}{reverse}\PY{o}{=}\PY{k+kc}{True}\PY{p}{)}
                 \PY{n}{weight} \PY{o}{=} \PY{p}{[}\PY{n}{s} \PY{o}{+} \PY{n}{d} \PY{k}{for} \PY{n}{s}\PY{p}{,} \PY{n}{d} \PY{o+ow}{in} \PY{n+nb}{zip}\PY{p}{(}\PY{n}{schur\PYZus{}delta\PYZus{}sorted}\PY{p}{,} \PY{n}{delta}\PY{p}{)}\PY{p}{]}
                 \PY{k}{return} \PY{p}{(}\PY{n}{ind}\PY{p}{,} \PY{n}{dimension}\PY{p}{(}\PY{n+nb}{tuple}\PY{p}{(}\PY{n}{weight}\PY{p}{)}\PY{p}{,} \PY{n}{n}\PY{p}{)}\PY{p}{)}
             \PY{k}{else}\PY{p}{:}
                 \PY{k}{return} \PY{k+kc}{None}
\end{Verbatim}

    \begin{Verbatim}[commandchars=\\\{\}]
{\color{incolor}In [{\color{incolor}5}]:} \PY{n}{R} \PY{o}{=} \PY{n}{SymmetricFunctions}\PY{p}{(}\PY{n}{QQ}\PY{p}{)}
         \PY{n}{s} \PY{o}{=} \PY{n}{R}\PY{o}{.}\PY{n}{schur}\PY{p}{(}\PY{p}{)}
         \PY{n}{r} \PY{o}{=} \PY{l+m+mi}{3} \PY{c+c1}{\PYZsh{}dealing with planes}
         \PY{n}{d} \PY{o}{=} \PY{n}{binomial}\PY{p}{(}\PY{n}{r}\PY{o}{+}\PY{l+m+mi}{2}\PY{p}{,}\PY{l+m+mi}{3}\PY{p}{)} \PY{c+c1}{\PYZsh{}d is the rank of Sym\PYZca{}3E}
         \PY{k}{for} \PY{n}{i} \PY{o+ow}{in} \PY{n+nb}{range}\PY{p}{(}\PY{n}{d}\PY{o}{+}\PY{l+m+mi}{1}\PY{p}{)}\PY{p}{:}
             \PY{c+c1}{\PYZsh{} In the following code, we print the Schur decomposition of \PYZbs{}}
             \PY{c+c1}{\PYZsh{} Wedge\PYZca{}iSym\PYZca{}3E\PYZbs{}otimes Sym\PYZca{}3E}
             \PY{n}{schur} \PY{o}{=} \PY{n}{s}\PY{p}{(}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{*}\PY{n}{i}\PY{p}{)}\PY{p}{(}\PY{n}{s}\PY{p}{[}\PY{l+m+mi}{3}\PY{p}{]}\PY{p}{)} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{3}\PY{p}{]}
             \PY{n}{part\PYZus{}list} \PY{o}{=} \PY{n+nb}{list}\PY{p}{(}\PY{p}{)}
             \PY{n}{coh\PYZus{}dict} \PY{o}{=} \PY{n+nb}{dict}\PY{p}{(}\PY{p}{)}
             \PY{k}{for} \PY{n}{part} \PY{o+ow}{in} \PY{n}{schur}\PY{p}{:}
                 \PY{k}{if} \PY{n+nb}{len}\PY{p}{(}\PY{n}{part}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{)} \PY{o}{\PYZlt{}}\PY{o}{=} \PY{n}{r}\PY{p}{:} 
                     \PY{c+c1}{\PYZsh{} print(f\PYZdq{}Working on \PYZob{}part[0]\PYZcb{}...\PYZdq{})}
                     \PY{n}{part\PYZus{}list}\PY{o}{.}\PY{n}{append}\PY{p}{(}\PY{n}{part}\PY{p}{)}
                     \PY{n}{coh} \PY{o}{=} \PY{n}{calculate\PYZus{}cohomology}\PY{p}{(}\PY{n}{part}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{,} \PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{,} \PY{l+m+mi}{3}\PY{p}{,} \PY{l+m+mi}{10}\PY{p}{)}
                     \PY{k}{if} \PY{n}{coh}\PY{p}{:}
                         \PY{k}{if} \PY{n}{coh}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]} \PY{o+ow}{in} \PY{n}{coh\PYZus{}dict}\PY{p}{:}
                             \PY{n}{coh\PYZus{}dict}\PY{p}{[}\PY{n}{coh}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{]} \PY{o}{+}\PY{o}{=} \PY{n}{part}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]} \PY{o}{*} \PY{n}{coh}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}
                         \PY{k}{else}\PY{p}{:}
                             \PY{n}{coh\PYZus{}dict}\PY{p}{[}\PY{n}{coh}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{]} \PY{o}{=} \PY{n}{part}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]} \PY{o}{*} \PY{n}{coh}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}
                         \PY{n+nb}{print}\PY{p}{(}\PY{n}{f}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+si}{\PYZob{}part[0]\PYZcb{}}\PY{l+s+s2}{ is regular: H\PYZca{}}\PY{l+s+si}{\PYZob{}coh[0]\PYZcb{}}\PY{l+s+s2}{ = }\PY{l+s+si}{\PYZob{}coh[1]\PYZcb{}}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}
                     \PY{c+c1}{\PYZsh{} else:}
                         \PY{c+c1}{\PYZsh{} print(\PYZdq{} irregular\PYZdq{})}
                     
             \PY{c+c1}{\PYZsh{} print(f\PYZdq{}The decomp of Wedge\PYZca{}\PYZob{}i\PYZcb{}Sym\PYZca{}3E otimes Sym\PYZca{}3E is \PYZob{}part\PYZus{}list\PYZcb{}\PYZdq{})}
             \PY{k}{for} \PY{n}{ind} \PY{o+ow}{in} \PY{n}{coh\PYZus{}dict}\PY{p}{:}
                 \PY{n+nb}{print}\PY{p}{(}\PY{n}{f}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{The dimension of H\PYZca{}}\PY{l+s+si}{\PYZob{}ind\PYZcb{}}\PY{l+s+s2}{(Wedge\PYZca{}}\PY{l+s+si}{\PYZob{}i\PYZcb{}}\PY{l+s+s2}{Sym\PYZca{}3E otimes Sym\PYZca{}3E) }\PY{l+s+se}{\PYZbs{}}
         \PY{l+s+s2}{is }\PY{l+s+si}{\PYZob{}coh\PYZus{}dict[ind]\PYZcb{}}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}
             \PY{k}{if} \PY{n}{coh\PYZus{}dict}\PY{p}{:}
                 \PY{n+nb}{print}\PY{p}{(}\PY{n}{f}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{And all the other cohomology of Wedge\PYZca{}}\PY{l+s+si}{\PYZob{}i\PYZcb{}}\PY{l+s+s2}{Sym\PYZca{}3E otimes }\PY{l+s+se}{\PYZbs{}}
         \PY{l+s+s2}{Sym\PYZca{}3E is 0}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}
             \PY{k}{else}\PY{p}{:}
                 \PY{n+nb}{print}\PY{p}{(}\PY{n}{f}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{All the cohomology of Wedge\PYZca{}}\PY{l+s+si}{\PYZob{}i\PYZcb{}}\PY{l+s+s2}{Sym\PYZca{}3E otimes Sym\PYZca{}3E is 0}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}
                 
             
             
             
\end{Verbatim}

    \begin{Verbatim}[commandchars=\\\{\}]
All the cohomology of Wedge\^{}0Sym\^{}3E otimes Sym\^{}3E is 0
All the cohomology of Wedge\^{}1Sym\^{}3E otimes Sym\^{}3E is 0
[8, 1] is regular: H\^{}7 = 10
The dimension of H\^{}7(Wedge\^{}2Sym\^{}3E otimes Sym\^{}3E) is 10
And all the other cohomology of Wedge\^{}2Sym\^{}3E otimes Sym\^{}3E is 0
[10, 1, 1] is regular: H\^{}7 = 55
The dimension of H\^{}7(Wedge\^{}3Sym\^{}3E otimes Sym\^{}3E) is 55
And all the other cohomology of Wedge\^{}3Sym\^{}3E otimes Sym\^{}3E is 0
All the cohomology of Wedge\^{}4Sym\^{}3E otimes Sym\^{}3E is 0
All the cohomology of Wedge\^{}5Sym\^{}3E otimes Sym\^{}3E is 0
[10, 9, 2] is regular: H\^{}14 = 10
The dimension of H\^{}14(Wedge\^{}6Sym\^{}3E otimes Sym\^{}3E) is 10
And all the other cohomology of Wedge\^{}6Sym\^{}3E otimes Sym\^{}3E is 0
All the cohomology of Wedge\^{}7Sym\^{}3E otimes Sym\^{}3E is 0
All the cohomology of Wedge\^{}8Sym\^{}3E otimes Sym\^{}3E is 0
[10, 10, 10] is regular: H\^{}21 = 1
The dimension of H\^{}21(Wedge\^{}9Sym\^{}3E otimes Sym\^{}3E) is 1
And all the other cohomology of Wedge\^{}9Sym\^{}3E otimes Sym\^{}3E is 0
[13, 10, 10] is regular: H\^{}21 = 220
The dimension of H\^{}21(Wedge\^{}10Sym\^{}3E otimes Sym\^{}3E) is 220
And all the other cohomology of Wedge\^{}10Sym\^{}3E otimes Sym\^{}3E is 0

    \end{Verbatim}

    \begin{Verbatim}[commandchars=\\\{\}]
{\color{incolor}In [{\color{incolor}6}]:} \PY{n}{R} \PY{o}{=} \PY{n}{SymmetricFunctions}\PY{p}{(}\PY{n}{QQ}\PY{p}{)}
        \PY{n}{s} \PY{o}{=} \PY{n}{R}\PY{o}{.}\PY{n}{schur}\PY{p}{(}\PY{p}{)}
        \PY{n}{r} \PY{o}{=} \PY{l+m+mi}{2} \PY{o}{+} \PY{l+m+mi}{1} \PY{c+c1}{\PYZsh{}dealing with planes}
        \PY{n}{n} \PY{o}{=} \PY{p}{(}\PY{n}{r} \PY{o}{+} \PY{l+m+mi}{2}\PY{p}{)} \PY{o}{*} \PY{p}{(}\PY{n}{r} \PY{o}{+} \PY{l+m+mi}{1}\PY{p}{)} \PY{o}{/}\PY{o}{/} \PY{l+m+mi}{2}
        \PY{n}{d} \PY{o}{=} \PY{n}{binomial}\PY{p}{(}\PY{n}{r}\PY{o}{+}\PY{l+m+mi}{2}\PY{p}{,}\PY{l+m+mi}{3}\PY{p}{)} \PY{c+c1}{\PYZsh{}d is the rank of Sym\PYZca{}3E}
        \PY{k}{for} \PY{n}{i} \PY{o+ow}{in} \PY{n+nb}{range}\PY{p}{(}\PY{n}{d}\PY{o}{+}\PY{l+m+mi}{1}\PY{p}{)}\PY{p}{:}
            \PY{c+c1}{\PYZsh{} In the following code, we print the Schur decomposition \PYZbs{}}
            \PY{c+c1}{\PYZsh{} of Wedge\PYZca{}iSym\PYZca{}3E\PYZbs{}otimes E\PYZbs{}otimes Q\PYZca{}*}
            \PY{n}{schur} \PY{o}{=} \PY{n}{s}\PY{p}{(}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{o}{*}\PY{n}{i}\PY{p}{)}\PY{p}{(}\PY{n}{s}\PY{p}{[}\PY{l+m+mi}{3}\PY{p}{]}\PY{p}{)} \PY{o}{*} \PY{n}{s}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}
            \PY{n}{part\PYZus{}list} \PY{o}{=} \PY{n+nb}{list}\PY{p}{(}\PY{p}{)}
            \PY{n}{coh\PYZus{}dict} \PY{o}{=} \PY{n+nb}{dict}\PY{p}{(}\PY{p}{)}
            \PY{k}{for} \PY{n}{part} \PY{o+ow}{in} \PY{n}{schur}\PY{p}{:}
                \PY{k}{if} \PY{n+nb}{len}\PY{p}{(}\PY{n}{part}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{)} \PY{o}{\PYZlt{}}\PY{o}{=} \PY{n}{r}\PY{p}{:} 
                    \PY{c+c1}{\PYZsh{} print(f\PYZdq{}Working on \PYZob{}part[0]\PYZcb{}...\PYZdq{})}
                    \PY{n}{part\PYZus{}list}\PY{o}{.}\PY{n}{append}\PY{p}{(}\PY{n}{part}\PY{p}{)}
                    \PY{n}{coh} \PY{o}{=} \PY{n}{calculate\PYZus{}cohomology}\PY{p}{(}\PY{n}{part}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{,} \PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{o}{*}\PY{p}{(}\PY{n}{n}\PY{o}{\PYZhy{}}\PY{n}{r}\PY{o}{\PYZhy{}}\PY{l+m+mi}{1}\PY{p}{)}\PY{o}{+}\PY{p}{[}\PY{o}{\PYZhy{}}\PY{l+m+mi}{1}\PY{p}{]}\PY{p}{,} \PYZbs{}
                                               \PY{n}{r}\PY{p}{,} \PY{n}{n}\PY{p}{)}
                    \PY{k}{if} \PY{n}{coh}\PY{p}{:}
                        \PY{k}{if} \PY{n}{coh}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]} \PY{o+ow}{in} \PY{n}{coh\PYZus{}dict}\PY{p}{:}
                            \PY{n}{coh\PYZus{}dict}\PY{p}{[}\PY{n}{coh}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{]} \PY{o}{+}\PY{o}{=} \PY{n}{part}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]} \PY{o}{*} \PY{n}{coh}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}
                        \PY{k}{else}\PY{p}{:}
                            \PY{n}{coh\PYZus{}dict}\PY{p}{[}\PY{n}{coh}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{]} \PY{o}{=} \PY{n}{part}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]} \PY{o}{*} \PY{n}{coh}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}
                        \PY{n+nb}{print}\PY{p}{(}\PY{n}{f}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+si}{\PYZob{}part[0]\PYZcb{}}\PY{l+s+s2}{ is regular: H\PYZca{}}\PY{l+s+si}{\PYZob{}coh[0]\PYZcb{}}\PY{l+s+s2}{ = }\PY{l+s+si}{\PYZob{}coh[1]\PYZcb{}}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}
                    \PY{c+c1}{\PYZsh{} else:}
                        \PY{c+c1}{\PYZsh{} print(\PYZdq{} irregular\PYZdq{})}
                    
            \PY{c+c1}{\PYZsh{} print(f\PYZdq{}The decomp of Wedge\PYZca{}\PYZob{}i\PYZcb{}Sym\PYZca{}3E otimes E otimes Q\PYZca{}* is \PYZbs{}}
            \PY{c+c1}{\PYZsh{} \PYZob{}part\PYZus{}list\PYZcb{}\PYZdq{})}
            \PY{k}{for} \PY{n}{ind} \PY{o+ow}{in} \PY{n}{coh\PYZus{}dict}\PY{p}{:}
                \PY{n+nb}{print}\PY{p}{(}\PY{n}{f}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{The dimension of H\PYZca{}}\PY{l+s+si}{\PYZob{}ind\PYZcb{}}\PY{l+s+s2}{(Wedge\PYZca{}}\PY{l+s+si}{\PYZob{}i\PYZcb{}}\PY{l+s+s2}{Sym\PYZca{}3E otimes E }\PY{l+s+se}{\PYZbs{}}
        \PY{l+s+s2}{otimes Q\PYZca{}*) is }\PY{l+s+si}{\PYZob{}coh\PYZus{}dict[ind]\PYZcb{}}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}
            \PY{k}{if} \PY{n}{coh\PYZus{}dict}\PY{p}{:}
                \PY{n+nb}{print}\PY{p}{(}\PY{n}{f}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{And all the other cohomology of Wedge\PYZca{}}\PY{l+s+si}{\PYZob{}i\PYZcb{}}\PY{l+s+s2}{Sym\PYZca{}3E }\PY{l+s+se}{\PYZbs{}}
        \PY{l+s+s2}{otimes E otimes Q\PYZca{}* is 0}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}
            \PY{k}{else}\PY{p}{:}
                \PY{n+nb}{print}\PY{p}{(}\PY{n}{f}\PY{l+s+s2}{\PYZdq{}}\PY{l+s+s2}{All the cohomology of Wedge\PYZca{}}\PY{l+s+si}{\PYZob{}i\PYZcb{}}\PY{l+s+s2}{Sym\PYZca{}3E otimes E }\PY{l+s+se}{\PYZbs{}}
        \PY{l+s+s2}{otimes Q\PYZca{}* is 0}\PY{l+s+s2}{\PYZdq{}}\PY{p}{)}
                
\end{Verbatim}

    \begin{Verbatim}[commandchars=\\\{\}]
[1] is regular: H\^{}1 = 1
The dimension of H\^{}1(Wedge\^{}0Sym\^{}3E otimes E otimes Q\^{}*) is 1
And all the other cohomology of Wedge\^{}0Sym\^{}3E otimes E otimes Q\^{}* is 0
All the cohomology of Wedge\^{}1Sym\^{}3E otimes E otimes Q\^{}* is 0
All the cohomology of Wedge\^{}2Sym\^{}3E otimes E otimes Q\^{}* is 0
All the cohomology of Wedge\^{}3Sym\^{}3E otimes E otimes Q\^{}* is 0
All the cohomology of Wedge\^{}4Sym\^{}3E otimes E otimes Q\^{}* is 0
All the cohomology of Wedge\^{}5Sym\^{}3E otimes E otimes Q\^{}* is 0
All the cohomology of Wedge\^{}6Sym\^{}3E otimes E otimes Q\^{}* is 0
[10, 9, 3] is regular: H\^{}15 = 10
The dimension of H\^{}15(Wedge\^{}7Sym\^{}3E otimes E otimes Q\^{}*) is 10
And all the other cohomology of Wedge\^{}7Sym\^{}3E otimes E otimes Q\^{}* is 0

    \end{Verbatim}


    

==> revision.tex <==
The complement $R$ of $\mathcal P^0_5$ in $\mathcal P_5$ is stratified by the following subsets $R_4, R_3, R_2, R_1$, where $R_i$ parametrizes $(L, P_4)\in R$ such that the residual $Q$ is of rank $i$.
        
         \textbf{Analysis of $R_4$.} The stratum $R_4$ parametrizes $(L, P_4)\in \mathcal P_5$ such that  $Q$ is singular at one point (equivalently, the rank of $Q$ is $4$) and that $L$ contains the singular point of $Q$. In this case, $Q$ is a cone from its singular point over a smooth quadric surface. 
        \begin{sublemma}\label{LmmLocusOfSimpleSingularQuadric}
            For any $3$-dimensional linear subspace $L$ contained in $Y$, the set of $4$-dimensional subspaces $P_4\subset \mathbb P^9$ containing $L$ such that $Q$ has a single singular point lying on $L$ has codimension at least $2$ in $\mathbb P^5=$\{$4$-dimensional subspaces $P_4\subset \mathbb P^9$ containing $L$\}.
        \end{sublemma}
        \begin{proof}
            Without loss of generality, let us assume $L=\{(x_0,\ldots, x_3, 0,\ldots, 0)\}\subset \mathbb P^9$. The fact that $L\subset Y$ implies that the defining equation of $Y$ is of the form
            \[
            f(x_0,\ldots, x_9)=\sum_{i=4}^9 x_iQ_i(x_0, \ldots, x_9),
            \]
            where $Q_i$ is a quadratic polynomial in the variables $x_0, \ldots, x_9$, for each $i\in \{4,\ldots, 9\}$. Let $\mathbf a:=(a_0, a_1, \ldots, a_5)\in \mathbb P^5$. Then $\mathbf a$ determines a dimension $4$ linear subspace $P_4$ containing $L$ as 
            \[
            P_4=\{(x_0, x_1, x_2, x_3, ta_0, ta_1,\ldots, ta_5): (x_0, x_1, x_2, x_3, t)\in \mathbb P^4\}.
            \]
            The corresponded residual quadric hypersuface $Q_{\mathbf a}$ is thus defined by 
            \[
            Q_{\mathbf a}(x_0, x_1, x_2, x_3, t)=\sum_{i=4}^9 a_{i-4} Q_i(x_0, x_1, x_2, x_3, ta_0, ta_1,\ldots, ta_5).
            \]
            We can identify the quadratic form $Q_{\mathbf a}(x_0, x_1, x_2, x_3, t)$ with a $5\times 5$ symmetric matrix that we still denote as $Q_{\mathbf a}$. Viewed as a function of $\mathbf a\in \mathbb P^5$, the matrix $Q_{\mathbf a}$ is a section of $\mathrm{Sym}^2(\mathcal O(1)_{\mathbb P^5}\oplus \mathcal O_{\mathbb P^5}^4)\otimes \mathcal O_{\mathbb P^5}(1)$, and thus the locus of $\mathbf a\in\mathbb P^5$ where $Q_{\mathbf a}$ degenerates is a degree $7$ hypersurface in $\mathbb P^5$. On the other hand, the quadratic polynomial of $Q_{\mathbf a}\cap L$ is $Q_{\mathbf a}(x_0, x_1, x_2, x_3, t=0)$, which, viewed as a $4\times 4$ symmetric matrix varing with $\mathbf a$, is a section of $\mathrm{Sym}^2( \mathcal O_{\mathbb P^5}^4)\otimes \mathcal O_{\mathbb P^5}(1)$, so that the degenerate locus of  $Q_{\mathbf a}\cap L$ is of degree $4$. Therefore, there exists a point $\mathbf a\in \mathbb P^5$ such that $Q_{\mathbf a}$ is singular whereas $Q_{\mathbf a}\cap L$ is smooth. Therefore, the locus of $\mathbf a\in\mathbb P^5$ such that $Q_{\mathbf a}$ is singular at exactly one point and that this point lies in $L$ is strictly contained, as a closed subset, in the locus where $Q_{\mathbf a}$ is singular at only one point. The latter locus is of codimension $1$ in $\mathbb P^5$ since it is defined by the vanishing of the determinant of the matrix $Q_{\mathbf a}$. Hence, the set of $4$-dimensional subspaces $P_4\subset \mathbb P^9$ containing $L$ such that $Q$ has a single singular point lying on $L$ has codimension at least $2$ in $\mathbb P^5$, as desired.
        \end{proof}
        \begin{sublemma}\label{LmmFiberOverASimpleSingularQuadric}
            The fiber of $\tilde f: \tilde F_{3,1}(Y)\to \mathcal P_5$ over an element $(L,P_4)$ such that the corresponding residual quadric $Q$ has only one singularities is isomorphic to the union 
            \[
            \mathcal P_2^*\cup \mathcal P_2^*,
            \]
            where $\mathcal P_2^*$ is a $\mathbb P^2$-bundle over $\mathbb P^1$, and the two $\mathcal P_2^*$ intersect at a smooth quadric surface.
        \end{sublemma}
        \begin{proof}
            The singular quadric hypersurface $Q$ is a cone from its only singular point $y$ over a smooth quadric surface $Q'$. Each line in $Q'$, together with $x$ determines a plane, and every line in $Q$ lies in some of these planes. There are two pencils of lines in $Q'$, each of which induces a pencil of planes in $Q'$. Each plane contains a $\mathbb P^2$ of lines. Hence, the lines in $Q$ is the union of two $\mathbb P^2$-bundles over $\mathbb P^1$. The intersection of these $\mathbb P^2$-bundles is the set of lines in $Q$ that pass through the singular point $y$, which is in turn isomorphic to $Q'$. 
        \end{proof}
        Sublemma~\ref{LmmLocusOfSimpleSingularQuadric} implies that $R_4\subset \mathcal P_5$ is of codimension at least $2$. Sublemma~\ref{LmmFiberOverASimpleSingularQuadric} shows that the dimension of the fiber of $\tilde f$ over $R_4$ is $3$, the same with that of the general fiber of $\tilde f: \tilde F_{3,1}(Y)\to \mathcal P_5$. Hence, the codimension of $\tilde f^{-1}(R_4)$ is at least $2$. This complete the analysis of $R_4$.
        
        \textbf{Analysis of $R_3$.} The stratum $R_3$ parametrizes $(L, P_4)\in \mathcal P_5$ such that $Q$ is of rank $3$. In this case, $Q$ is singular along a line and is a cone from one of its singular point over a quadric cone surface.
        \begin{sublemma}\label{LmmCodimOfStrata}
            The stratum $R_3, R_2, R_1$ is of codimension $3, 6, 10$ in $\mathcal P_5$. In particular, $R_1=\emptyset$.
        \end{sublemma}
        \begin{proof}
            Let $\mathcal E_4$ and $\mathcal Q_6$ be the tautological subbundle, respectively, tautological quotient bundle over $F_3(Y)$. Then $\mathcal P_5$ is nothing but the projectivization of $\mathcal Q_6$. Let $\mathcal H$ be the Hopf bundle of $\mathbb P(\mathcal Q_6)$, which is a subbundle of $\pi^*\mathcal Q_6$. Let $\mathcal F_5$ be the kernel of the composite of the canonical maps $V_{10}\to \pi_*\mathcal Q_6\to \pi_*\mathcal Q_6/\mathcal H$, where the first map is the universal quotient map of bundles of $\mathbb P(\mathcal Q_6)$. Then there is a natural exact sequence of vector bundles on $\mathbb P(\mathcal Q_6)$:
            \[
            0\to \pi^*\mathcal E_4\to \mathcal F_5\to \mathcal H\to 0.
            \]
            The defining equation of $Y\subset \mathbb P^9$ gives a section of the bundle $\mathrm{Sym}^3\mathcal F_5^*$ whose image in $\pi^*\mathrm{Sym}^3\mathcal E_4^*$ vanishes since the fibers of $\mathbb P(\mathcal E_4)$ are by definition $3$-dimensional linear subspaces in $Y$. Hence, the universal residual quadric hypersurface is defined by a section of the bundle $\mathrm{Sym}^2\mathcal F_5^*\otimes \mathcal H^*$. Notice that $\mathrm{Sym}^2\mathcal F_5^*\otimes \mathcal H^*$ is generated by global sections. Since $Y$ is general, the locus where such a quadratic form is of rank $\leq r$ is $\binom{6-r}{2}$, for $r\in\{0,\ldots, 4\}$, as desired.
        \end{proof}
        \begin{sublemma}\label{LmmFiberOverR3}
            The fiber of $\tilde f: \tilde F_{3,1}(Y)\to \mathcal P_5$ over a point $(L, P_4)$ in $R_3$ is of dimension $3$.
        \end{sublemma}
        \begin{proof}
            The residual quadric hypersurface $Q$ is singular along a line and is a cone from one of its singular point over a quadric cone surface. By the same argument as in Sublemma~\ref{LmmFiberOverASimpleSingularQuadric}, the variety of lines in $Q$ is isomorphic to a $\mathbb P^2$-bundle over a smooth conic, thus has dimension $3$.
        \end{proof}
        By Sublemma~\ref{LmmCodimOfStrata} and Sublemma~\ref{LmmFiberOverR3}, the codimension of $\tilde f^{-1}(R_3)$ is $3$. This complete the analysis of $R_3$.
        
        \textbf{Analysis of $R_2$.} The stratum $R_2$ parametrizes $(L, P_4)\in \mathcal P_5$ such that $Q$ is of rank $2$. In this case, $Q$ is a union of two $3$-dimensional linear subspaces intersecting along a plane. It is clear that in this case, the variety of lines in $Q$ is isomorphic to the union of two $\mathrm{Gr}(2,4)$ intersecting along a $\mathbb P^2$. Hence, the dimension of fibers of $\tilde f$ over $R_2$ is $4$. By Sublemma~\ref{LmmCodimOfStrata}, the codimension of $\tilde f^{-1}(R_2)$ is $5$. This complete the analysis of $R_2$.
        
        \textbf{Analysis of $R_1$.} The stratum $R_1$ parametrizes $(L, P_4)\in \mathcal P_5$ such that $Q$ is of rank $1$. By Sublemma~\ref{LmmCodimOfStrata}, this case does not happen.
        
        The case where $Q$ is of rank $0$ does not happen, since in this case, $P_4$ is contained in $Y$, which cannot happen if $Y$ is a general cubic eightfold.

